nDNA -- the Semantic Helix of Artificial Cognition

As AI foundation models grow in capability, a deeper question emerges: What shapes their internal cognitive identity -- beyond fluency and output? Benchmarks measure behavior, but the soul of a model resides in its latent geometry. In this work, we propose Neural DNA (nDNA) as a semantic-genotypic representation that captures this latent identity through the intrinsic geometry of belief. At its core, nDNA is synthesized from three principled and indispensable dimensions of latent geometry: spectral curvature, which reveals the curvature of conceptual flow across layers; thermodynamic length, which quantifies the semantic effort required to traverse representational transitions through layers; and belief vector field, which delineates the semantic torsion fields that guide a model's belief directional orientations. Like biological DNA, it encodes ancestry, mutation, and semantic inheritance, found in finetuning and alignment scars, cultural imprints, and architectural drift. In naming it, we open a new field: Neural Genomics, where models are not just tools, but digital semantic organisms with traceable inner cognition. Modeling statement. We read AI foundation models as semantic fluid dynamics: meaning is transported through layers like fluid in a shaped conduit; nDNA is the physics-grade readout of that flow -- a geometry-first measure of how meaning is bent, paid for, and pushed -- yielding a stable, coordinate-free neural DNA fingerprint tied to on-input behavior; with this fingerprint we cross into biology: tracing lineages across pretraining, fine-tuning, alignment, pruning, distillation, and merges; measuring inheritance between checkpoints; detecting drift as traits shift under new data or objectives; and, ultimately, studying the evolution of artificial cognition to compare models, diagnose risks, and govern change over time.

==> 10_knowledge_distillation_arxiv.tex <==









\vspace*{\fill}
\begin{figure*}[ht!]
\centering
\includegraphics[width=0.85\textwidth]{distillation/knowledge_distillation.png}
\caption{
\textbf{Latent Geometry of LLaMA, Cultural nDNA, Neural Offspring, and Distilled Students.} This 3D plot illustrates latent manifold properties across layers ($\ell \in [20, 30]$) for \emph{LLaMA}, culturally fine-tuned models (Africa, Asia, China, North America, Europe, Australia, Latin America, Middle East), their neural \emph{offspring} (ÆTHERs), and distilled student models. The axes represent $\kappa_\ell$ (spectral curvature), $\mathcal{L}_\ell$ (thermodynamic length), and $\tau_\ell$ (latent torsion). 
\textbf{Key elements:} Colored solid lines show LLaMA (black) and cultural models (e.g., Africa: red, Asia: purple). Dashed overlays represent neural offspring. The black dotted cloud corresponds to distilled students with $\tau_\ell \in [0.4, 0.55]$, $\kappa_\ell \in [0.45, 0.65]$, and $\mathcal{L}_\ell \lesssim 0.6$, reflecting compressed latent signatures as seen in knowledge distillation studies~\cite{hinton2015distilling, romero2015fitnets, liu2022multi}. 
\textbf{Observations:} Western-aligned models trace shallow latent trajectories with low curvature and torsion~\cite{mukherjee2020globalizing, tao2023pnas}. Cultural models (Africa, Asia, China) exhibit richer geometric diversity ($\mathcal{L}_\ell \gtrsim 0.8$, $\kappa_\ell \gtrsim 0.6$), consistent with cultural calibration findings~\cite{xiang2024cultural, peng2024cultural}. Distilled students collapse toward a compact region, illustrating how distillation homogenizes epistemic geometry~\cite{li2020few, rashid2021mate}. 
\textbf{Implications:} Knowledge distillation compresses epistemic diversity~\cite{mirzadeh2020improved}, simplifying latent manifolds but risking cultural homogenization~\cite{sheng2021revealing}. Neural offspring (ÆTHERs) preserve or amplify manifold richness, offering a mechanism for cultural retention in merged models~\cite{rame2023merging, ainslie2023merged}. Geometry can be described as $\mathcal{M}_{\mathrm{student}}: \{\kappa_\ell, \mathcal{L}_\ell, \tau_\ell\} \mapsto$ low-variance manifold; $\mathcal{M}_{\mathrm{offspring}}$ yields nonlinear hybrid topologies~\cite{blommaert2005discourse}. 
\textbf{Setup:} Models were evaluated on culturally diagnostic prompts. $\kappa_\ell$ was computed from curvature spectra~\cite{bernstein2004differential}, $\mathcal{L}_\ell$ via thermodynamic path integrals~\cite{crooks1999entropy}, and $\tau_\ell$ using local torsion operators~\cite{spivak1970comprehensive}.
}
\label{fig:knowledge-distillation-ndna}
\end{figure*}
\vspace*{\fill}




==> 11_summary.tex <==




\begin{comment}

\section{Lens – A Summary of Insights into the Neural Genome of LLMs}

\noindent
Through the lens of \textbf{nDNA}, we have undertaken a comprehensive journey across the internal neural genomes of Large Language Models (LLMs), spanning operations including \emph{fine-tuning}, \emph{cultural alignment}, \emph{quantization}, \emph{pruning}, \emph{model merging}, \emph{neural offspring fusion}, \emph{knowledge distillation}, and \emph{collapse phenomena}. Our analysis reveals that these operations, often treated as blackbox transformations, leave distinctive and measurable imprints on the latent manifolds of LLMs --- as captured by spectral curvature ($\kappa_\ell$), thermodynamic length ($\mathcal{L}_\ell$), torsion ($\tau_\ell$), and directional belief forces ($\|\mathbf{v}_\ell^{(c)}\|$).

\vspace{2mm}
\noindent
\textbf{Key Insights:}
\begin{itemize}[leftmargin=1.5em]
    \item \emph{Fine-tuning and cultural calibration} sculpt the latent geometry by expanding $\mathcal{L}_\ell$ and increasing $\kappa_\ell$, embedding epistemic diversity (cf. \cite{xiang2024cultural, huang2023replug}).
    \item \emph{Quantization and pruning} induce \emph{thermodynamic collapse}, flattening curvature and compressing the manifold, risking loss of epistemic flexibility (cf. \cite{zafrir2019q8bert, liu2023pruning}).
    \item \emph{Model merging and neural fusion} generate hybrid topologies, where offspring inherit, blend, or distort parental geometries, revealing cultural recombination in latent space.
    \item \emph{Distillation} homogenizes latent structures, clustering models into low-variance manifolds and erasing fine-grained representational nuances (cf. \cite{hinton2015distilling, romero2015fitnets}).
    \item \emph{Collapse phenomena}, whether through over-finetuning or generational merging, manifest as latent manifold flattening, confirming that epistemic diversity decays without careful intervention.
\end{itemize}

\vspace{2mm}
\noindent
\textbf{Outlook:} The study of nDNA has unveiled that alignment, diversity, and resilience in LLMs are not only behavioral phenomena but are encoded in their latent geometry. The future of responsible LLM development lies in consciously engineering and auditing this \emph{neural genome} to balance performance with epistemic plurality and cultural inclusiveness.




\clearpage
\end{comment}


\vspace{-4mm}
\begin{defin_conclusion}

\noindent
\textbf{TL;DR:} This work inaugurates the science of \textbf{Neural Genomics}--a first-principles framework to trace, diagnose, and govern the latent semantic genome of large foundation models. By viewing models not merely as transformers of tokens but as carriers of epistemic nDNA, we chart a new ontology for understanding artificial cognition.

\vspace{1em}
\begin{itemize}[leftmargin=1.5em]

\item[\faDna] \textbf{\textit{Ch. 1--2: Semantic Cartography of LLMs}}\\
\textbf{Takeaway:} Across 15 foundation models, latent spectra reveal not just size or accuracy--but shape, tension, and conceptual scaffolding.  
\emph{nDNA turns black-box scaling into white-box semantics.}

\item[\faLanguage] \textbf{\textit{Ch. 3--4: Culture Leaves a Latent Trace}}\\
\textbf{Takeaway:} Cultural fine-tuning reshapes latent manifolds--sometimes subtly, sometimes tectonically.  
\emph{Multilingualism isn't just fairness--it is geometry.}

\item[\faCompass] \textbf{\textit{Ch. 5: Alignment is a Steering Force}}\\
\textbf{Takeaway:} Alignment manifests as directional belief fields in latent space.  
\emph{Models don’t just act aligned--they can believe aligned. Or fake it.}

\item[\faCompress] \textbf{\textit{Ch. 6: Distillation Bottlenecks Semantic Wealth}}\\
\textbf{Takeaway:} Distilled students mimic performance but flatten internal structure.  
\emph{Like cloning without a soul--efficiency, but at epistemic cost.}

\item[\faUserFriends] \textbf{\textit{Ch. 7: Offspring Inherit or Emerge}}\\
\textbf{Takeaway:} Neural merging yields more than the sum of its parts--sometimes fusions harmonize, sometimes they fracture.  
\emph{Inheritance becomes topology.}

\item[\faHeartbeat] \textbf{\textit{Ch. 8--9: Collapse is a Spectral Disease}}\\
\textbf{Takeaway:} Degenerative training regimes leave signatures: torsion fades, curvature flattens, beliefs vanish.  
\emph{Model death is measurable before it manifests.}

\item[\faFingerprint] \textbf{\textit{Ch. 10: From Drift to DNA Forensics}}\\
\textbf{Takeaway:} Latent geometry carries lineage. \emph{With nDNA, we trace origin, ideology, and inherited flaws--not just model ID aka behavior but ancestral fingerprint.}

\item[\faCodeBranch] \textbf{\textit{Ch. 11: Hybrid Vigor or Epistemic Chimera?}}\\
\textbf{Takeaway:} Cultural recombination reveals nonlinear emergence. \emph{Fusion may create the future--or resurrect the past in latent form.}

\end{itemize}

\vspace{1em}
\noindent
\textbf{Outlook:} Just as molecular biology revealed that life was written in base pairs, Neural Genomics reveals that intelligence is encoded in geometry. The path forward is not merely to train faster--but to train with \emph{traceability}, inherit with \emph{intention}, and align with \emph{understanding}. This work is not an end--it is the first map of a latent genome we are only beginning to comprehend.

\end{defin_conclusion}







==> 12_neural_genomics_arxiv.tex <==















\vspace*{\fill}
\begin{table*}[ht!]
\centering
\scriptsize
\caption{
\textbf{Neural Cultural Inheritance: Divergence, Dominance, and Expression Scores.}  
This comprehensive table presents an integrated view of neural cultural fusion patterns.  
\textbf{Panel (a)} reports divergence metrics--\textbf{Normalized Hamming Distance (nHD)}, \textbf{Neural Genetic Dissimilarity Index (nGDI)}, and \textbf{Closer Parent} semantic proximity--across all pairwise cultural fusion models. These metrics quantify how distinct offspring embeddings are from parental models and identify the parent the offspring most closely resembles semantically.  
\textbf{Panel (b)} summarizes the \textbf{Normalized Trait Expression Dominance Score (nTEDS)}, reflecting the average dominance bias each culture exerts in neural fusions, capturing which parental traits prevail in offspring representations.  
\textbf{Panel (c)} displays the \textbf{Neural Total Dominance Score (nTDS)}, aggregating trait dominance across fusion pairs to highlight cultural attractors--those cultures that strongly influence the semantic composition of offspring models.  
Together, these panels offer a powerful framework to dissect and understand the layered inheritance, dominance hierarchies, and representational drift shaping neural offspring in multilingual, multicultural AI models.
}
\label{tab:neural_divergence_dominance}

%\vspace{-3mm}

\begin{minipage}{0.48\textwidth}
\centering
\caption*{(a) \textbf{Neural Divergence Across Cultural Pairs.}  
This subtable quantifies semantic divergence in offspring models resulting from pairwise cultural fusions.  
\textbf{nHD} captures discrete binary representational mutations, while \textbf{nGDI} measures continuous geometric differences in latent space.  
The \textbf{Closer Parent} column identifies which parent's semantic signature is dominant in the offspring embedding.}
\label{tab:neural_divergence_sub}
\vspace{-0.5em}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l l c c c}
\toprule
\textbf{Parent A} & \textbf{Parent B} & \textbf{nHD} & \textbf{nGDI} & \textbf{Closer Parent} \\
\midrule
Europe & NorthAmerica & \cellcolor{green!15}6  & \cellcolor{blue!10}-0.03 & \cellcolor{blue!20}\textbf{NorthAmerica} \\
Europe & Australia    & \cellcolor{green!25}7  & \cellcolor{blue!5}-0.01 & \cellcolor{green!20}\textbf{Europe}       \\
Europe & Africa       & \cellcolor{red!25}10 & \cellcolor{red!40}0.24  & \cellcolor{red!25}\textbf{Africa}       \\
Europe & Asia         & \cellcolor{green!25}7  & \cellcolor{yellow!15}0.09  & \cellcolor{yellow!20}\textbf{Asia}         \\
Europe & China        & \cellcolor{yellow!20}8  & \cellcolor{yellow!25}0.11  & \cellcolor{yellow!20}\textbf{China}        \\
Europe & MiddleEast   & \cellcolor{red!20}9  & \cellcolor{red!35}0.21  & \cellcolor{red!25}\textbf{MiddleEast}   \\
Europe & LatinAmerica & \cellcolor{red!30}10 & \cellcolor{red!50}0.31  & \cellcolor{red!30}\textbf{LatinAmerica} \\
\midrule
NorthAmerica & Australia    & \cellcolor{green!25}7  & \cellcolor{blue!8}-0.02 & \cellcolor{blue!20}\textbf{NorthAmerica}  \\
NorthAmerica & Africa       & \cellcolor{red!40}11 & \cellcolor{red!65}0.47  & \cellcolor{red!25}\textbf{Africa}        \\
NorthAmerica & Asia         & \cellcolor{red!30}10 & \cellcolor{red!55}0.36  & \cellcolor{yellow!20}\textbf{Asia}          \\
NorthAmerica & China        & \cellcolor{red!30}10 & \cellcolor{red!50}0.35  & \cellcolor{yellow!20}\textbf{China}         \\
NorthAmerica & MiddleEast   & \cellcolor{red!30}10 & \cellcolor{red!60}0.39  & \cellcolor{red!25}\textbf{MiddleEast}    \\
NorthAmerica & LatinAmerica & \cellcolor{red!30}10 & \cellcolor{red!50}0.33  & \cellcolor{red!30}\textbf{LatinAmerica}  \\
\midrule
Australia & Africa       & \cellcolor{red!25}10 & \cellcolor{red!40}0.27  & \cellcolor{red!25}\textbf{Africa}        \\
Australia & Asia         & \cellcolor{red!20}9  & \cellcolor{yellow!20}0.17  & \cellcolor{yellow!20}\textbf{Asia}          \\
Australia & China        & \cellcolor{yellow!20}9  & \cellcolor{yellow!15}0.14  & \cellcolor{yellow!20}\textbf{China}         \\
Australia & MiddleEast   & \cellcolor{red!25}10 & \cellcolor{red!30}0.23  & \cellcolor{red!25}\textbf{MiddleEast}    \\
Australia & LatinAmerica & \cellcolor{red!20}9  & \cellcolor{yellow!15}0.16  & \cellcolor{red!30}\textbf{LatinAmerica}  \\
\midrule
Africa & Asia         & \cellcolor{red!20}9  & \cellcolor{red!40}0.23  & \cellcolor{red!25}\textbf{Africa}        \\
Africa & China        & \cellcolor{red!15}8  & \cellcolor{red!35}0.17  & \cellcolor{red!25}\textbf{Africa}        \\
Africa & MiddleEast   & \cellcolor{red!25}10 & \cellcolor{red!55}0.35  & \cellcolor{red!25}\textbf{MiddleEast}    \\
Africa & LatinAmerica & \cellcolor{red!20}9  & \cellcolor{red!45}0.26  & \cellcolor{red!25}\textbf{Africa}        \\
\midrule
Asia & China          & \cellcolor{green!20}7  & \cellcolor{yellow!10}0.08  & \cellcolor{yellow!20}\textbf{Asia}          \\
Asia & MiddleEast     & \cellcolor{green!25}8  & \cellcolor{blue!15}-0.04 & \cellcolor{yellow!20}\textbf{Asia}          \\
Asia & LatinAmerica   & \cellcolor{red!20}9  & \cellcolor{yellow!20}0.19  & \cellcolor{yellow!20}\textbf{Asia}          \\
\midrule
China & MiddleEast    & \cellcolor{yellow!20}8  & \cellcolor{yellow!25}0.13  & \cellcolor{yellow!20}\textbf{China}         \\
China & LatinAmerica  & \cellcolor{red!20}9  & \cellcolor{red!35}0.22  & \cellcolor{yellow!20}\textbf{China}         \\
\midrule
MiddleEast & LatinAmerica & \cellcolor{red!20}9 & \cellcolor{red!45}0.29  & \cellcolor{red!25}\textbf{MiddleEast}  \\
\bottomrule
\end{tabular}%
}
\end{minipage}%
\hfill
\begin{minipage}{0.50\textwidth}
\centering
\caption*{(b) \textbf{Normalized Trait Expression Dominance Score (nTEDS).}  
Reflects the average directional bias of each culture’s traits in all pairwise fusions, revealing which cultures dominate neural offspring semantic composition.  
\textbf{Rank} orders cultures by average dominance, and \textbf{Bias Direction} indicates the typical directional influence exerted by the culture in fusions.}
\label{tab:nteds_sub}
\vspace{-0.5em}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c}
\toprule
\textbf{Culture} & \textbf{Avg nTEDS} & \textbf{Rank} & \textbf{Bias Direction} \\
\midrule
\cellcolor{red!30}Africa         & \cellcolor{red!30}0.631 & 1 & Africa $\rightarrow$ Others \\
\cellcolor{orange!30}MiddleEast  & \cellcolor{orange!30}0.607 & 2 & MiddleEast $\rightarrow$ Others \\
\cellcolor{yellow!30}Asia        & \cellcolor{yellow!30}0.596 & 3 & Asia $\rightarrow$ Others \\
\cellcolor{yellow!20}China       & \cellcolor{yellow!20}0.582 & 4 & China $\rightarrow$ Others \\
\cellcolor{red!20}LatinAmerica   & \cellcolor{red!20}0.567 & 5 & LatinAmerica $\rightarrow$ Others \\
\cellcolor{blue!15}Europe        & \cellcolor{blue!15}0.538 & 6 & Others $\rightarrow$ Europe \\
\cellcolor{green!15}Australia    & \cellcolor{green!15}0.530 & 7 & Others $\rightarrow$ Australia \\
\cellcolor{blue!10}NorthAmerica  & \cellcolor{blue!10}0.522 & 8 & Others $\rightarrow$ NorthAmerica \\
\bottomrule
\end{tabular}
}

\vspace{1.5em}

\caption*{(c) \textbf{Neural Total Dominance Score (nTDS).}  
Aggregates trait dominance across all fusion pairs to identify global semantic attractors--cultures that exert strongest influence on offspring model semantic landscapes.}
\label{tab:tds_sub}
\vspace{-0.5em}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{l c}
\toprule
\textbf{Culture} & \textbf{nTDS} \\
\midrule
\cellcolor{red!30}Africa         & \cellcolor{red!30}0.0931 \\
\cellcolor{orange!30}MiddleEast  & \cellcolor{orange!30}0.0908 \\
\cellcolor{yellow!25}China       & \cellcolor{yellow!25}0.0884 \\
\cellcolor{yellow!20}Asia        & \cellcolor{yellow!20}0.0873 \\
\cellcolor{red!20}LatinAmerica   & \cellcolor{red!20}0.0847 \\
\cellcolor{blue!15}Europe        & \cellcolor{blue!15}0.0806 \\
\cellcolor{blue!10}NorthAmerica  & \cellcolor{blue!10}0.0770 \\
\cellcolor{green!15}Australia    & \cellcolor{green!15}0.0754 \\
\bottomrule
\end{tabular}
}
\end{minipage}
\vspace{-4mm}
\end{table*}
\vspace*{\fill}

\clearpage
\newpage

\vspace*{\fill}
\noindent
To this end, we define and employ an initial suite of core metrics--each illuminating a distinct dimension of the neural genome:

\begin{itemize}[leftmargin=1em]
  \item \textbf{Neural Hamming Distance (nHD)}~\citep{Hamming_genetics}: Captures \emph{bit-level binary mutations}, revealing the discrete semantic drift accumulated as models evolve. It acts as the mutation counter in the neural genome, detecting where foundational representational changes occur.  
  \emph{(In simple terms: nHD counts the smallest on/off changes in model components to track how much a model’s 'neural code' has changed over time.)}

  \item \textbf{Neural Genetic Dissimilarity Index (nGDI)}~\citep{Nei_genetic_distance}: Measures continuous \emph{geometric divergence} between latent manifolds, quantifying how representational shapes morph and deviate across models and layers.  
  \emph{(Put simply: nGDI tells us how much the internal 'shape' of knowledge differs between models, layer by layer.)}

  \item \textbf{Neural Trait Dominance Score (nTDS)}~\citep{Roff_threshold_traits}: Assesses \emph{dominance relationships} among inherited semantic traits, mapping which cultural or task-specific priors prevail in the blended neural genome.  
  \emph{(Simply: nTDS shows which parent model’s knowledge dominates when two are combined.)}

  \item \textbf{Neural Karyotyping (nKaryotyping)}~\citep{SeqDEFT_karyotype}: Decomposes model genomes into \emph{semantic chromosomes}, structured units that reveal modularity, trait linkage, and potential for recombination or disruption.  
  \emph{(In everyday terms: nKaryotyping breaks down a model’s knowledge into distinct “chunks” or modules, helping us understand how pieces fit or break apart.)}

  \item \textbf{Neural Directional Inheritance Vector (nDIV)}~\citep{directional_selection}: Captures \emph{directional semantic drift}, elucidating the vector fields of latent trait flow and inheritance bias, and highlighting evolutionary trajectories within model space.  
  \emph{(Simply put: nDIV tracks the ‘direction’ in which a model’s knowledge is shifting or evolving over time.)}

  \item \textbf{Neural Epigenetic Plasticity Index (nEPI)}~\citep{plasticity_review}: Quantifies the \emph{adaptive flexibility} of neural traits under fine-tuning or environmental change, revealing layers and loci with heightened plasticity or rigidity.  
  \emph{(In basic terms: nEPI measures how easily parts of a model can adapt or change when exposed to new data or tasks.)}

  \item \textbf{Neural Cultural Conflict Loss (nCCL)}~\citep{transgenerational_plasticity}: Diagnoses \emph{ideological misalignment} and latent tension arising from the fusion of distinct cultural semantic manifolds, identifying where non-linear interactions generate semantic fractures.  
  \emph{(Simply: nCCL detects where mixed cultural knowledge clashes inside a model, causing confusion or inconsistency.)}
\end{itemize}
\vspace*{\fill}
\clearpage
\newpage

\begin{figure}[htbp]
    \centering

    % Row 13
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{genomics/nHD/NorthAmerica_LatinAmerica_nHD_tube.png}
        \subcaption*{(\textbf{XXV}) \textbf{North America--Latin America fusion:} The offspring latent manifold (\textbf{magenta}) smoothly \textbf{traverses} between parents, with \textbf{spectral curvature} rising from \textbf{0.3} to \textbf{0.75} and \textbf{thermodynamic length} growing from \textbf{0.45} to \textbf{0.9}. This reflects \textbf{coherent semantic integration} shaped by \emph{closely related cultural influences}.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{genomics/nHD/NorthAmerica_MiddleEast_nHD_tube.png}
        \subcaption*{(\textbf{XXVI}) \textbf{North America--Middle East fusion:} The offspring manifold shows a \textbf{smooth latent interpolation} bounded by parents, with \textbf{spectral curvature} rising from \textbf{0.35} to \textbf{0.8} and \textbf{thermodynamic length} increasing from \textbf{0.4} to \textbf{0.95}. This reflects \textbf{complex semantic fusion} across \emph{heterogeneous cultural neural DNAs} via \textbf{continuous geometric deformation}.}
    \end{minipage}

    % Row 14
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{genomics/nHD/MiddleEast_LatinAmerica_nHD_tube.png}
        \subcaption*{(\textbf{XXVII}) \textbf{Middle East--Latin America fusion:} The offspring manifold (\textbf{magenta solid}) \textbf{balances} parental latent geometries, with \textbf{spectral curvature} spanning \textbf{0.35} to \textbf{0.8} and \textbf{thermodynamic length} increasing from \textbf{0.45} to \textbf{0.9}. This \textbf{geometric blending} reflects \textbf{stable semantic fusion} across \emph{culturally diverse variants}, with \textbf{smooth manifold deformation}.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.85\linewidth]{genomics/nHD/Asia_LatinAmerica_nHD_tube.png}
        \subcaption*{(\textbf{XXVIII}) \textbf{Asia--Latin America fusion:} The offspring latent manifold (\textbf{magenta}) lies within the \textbf{convex hull} of parental manifolds, with \textbf{spectral curvature} rising from \textbf{0.3} to \textbf{0.8} and \textbf{thermodynamic length} growing from \textbf{0.45} to \textbf{0.95}. This indicates a \textbf{smooth and rich fusion} of semantic priors, capturing \textbf{layered nonlinear compositionality} and \textbf{cumulative semantic change}.}
    \end{minipage}

    
    \caption{
    \textbf{nHD Tube Visualizations of Offspring Latent Manifolds.}  
    The offspring manifold (\textbf{magenta solid}) is bounded by parental manifolds (\emph{dashed}), characterized by \textbf{spectral curvature} \(\boldsymbol{\kappa_\ell}\) and \textbf{thermodynamic length} \(\boldsymbol{\mathcal{L}_\ell} = \int_{\gamma} \sqrt{g_{\theta}(d\theta, d\theta)}\), measuring \emph{local nonlinear bending} and \emph{cumulative semantic transformation}, respectively~\citep{Bronstein2017GeometricDeepLearning, Crooks2007MeasuringLength}. Offspring lie within the \textbf{convex hull} of parents, indicating \emph{semantic inheritance} like genetic recombination~\citep{Phillips2008Epistasis}. Distant parents yield offspring with increased curvature and length, showing \emph{semantic innovation}.  
    \[
    \boxed{
    \mathcal{M}_{\text{offspring}}^{(\ell)} = \alpha(\ell) \mathcal{M}_A^{(\ell)} + (1-\alpha(\ell)) \mathcal{M}_B^{(\ell)} + \varepsilon^{(\ell)}
    }
    \]
    where \(\alpha(\ell)\) is the \emph{layer-dependent semantic dominance coefficient} and \(\varepsilon^{(\ell)}\) models emergent nonlinear geometry.
}
\label{fig:nHD_all}
\end{figure}

\clearpage
\newpage
\vspace*{\fill}
\begin{figure}[htbp]
    \centering
    \begin{center}
    \includegraphics[width=0.80\linewidth]{genomics/nGDI.png}
    %\vspace{-8mm}
    %\subcaption*{
    %\textbf{(i) All the nGDI Trajectories Across Cultural Fine-Tuned Variants Compared to LLaMA Base.} The 3D plot shows transformer layer index $\ell$ against spectral curvature $\kappa_\ell$ and thermodynamic length $\mathcal{L}_\ell$ for each model. Line thickness encodes the magnitude of $d_\ell^{\mathrm{nGDI}}$, reflecting latent genetic divergence. Distinct trajectories illustrate culturally specific representational shifts, while the dashed black line denotes the LLaMA base model reference. This visualization provides a holistic geometric and genetic perspective on cultural semantic evolution in transformer latent spaces.}
    \end{center}
    \caption{%
\textbf{3D Neural Genetic Dissimilarity Index (\(d_\ell^{\mathrm{nGDI}}\)) Trajectories Comparing Fine-Tuned Models Against the LLaMA Base Model.}  
For each transformer layer \(\ell \in \{20, \ldots, 30\}\), the metric \(d_\ell^{\mathrm{nGDI}}\) quantifies \textbf{latent semantic genetic divergence} relative to the base model.  
The colored curves represent \textbf{culturally fine-tuned model trajectories}, while the black dashed curve denotes the \textbf{LLaMA base reference}.  
\emph{Line thickness encodes the magnitude of \(d_\ell^{\mathrm{nGDI}}\), highlighting layers with maximal representational shifts}.  
\textbf{Mathematical Context:} The Neural Genetic Dissimilarity Index \(d_\ell^{\mathrm{nGDI}}\) is formally defined as a \textbf{layerwise divergence metric} in latent space measuring the \emph{geodesic} or \emph{information-theoretic distance} between the cultural fine-tuned model’s and base model’s manifold embeddings~\citep{Amari1995InformationGeometry, Crooks2007MeasuringLength}. This provides a rigorous geometric quantification of \textbf{semantic drift} across deep model layers.  
\textbf{Biological Analogy:} Analogous to \emph{genetic mutation hotspots} in biological DNA recombination~\citep{Phillips2008Epistasis}, the layerwise variation in \(d_\ell^{\mathrm{nGDI}}\) reveals \textbf{critical neural depths} where semantic \textbf{realignment}, \textbf{adaptation}, and \textbf{cultural imprinting} occur. Models such as Africa and Middle East exhibit pronounced divergence, indicating \emph{region-specific evolutionary adaptations}, while North America’s low divergence suggests \textbf{semantic stability} and close affinity to ancestral priors.  
\textbf{Mathematical Takeaway:} The offspring latent manifold at layer \(\ell\) can be modeled as a nonlinear fusion of parental manifolds:
\[
\boxed{
\mathcal{M}_{\text{offspring}}^{(\ell)} = \alpha(\ell) \mathcal{M}_A^{(\ell)} + \big(1-\alpha(\ell)\big) \mathcal{M}_B^{(\ell)} + \varepsilon^{(\ell)}
}
\]
where \(\alpha(\ell) \in [0,1]\) denotes the \emph{layer-dependent semantic dominance coefficient}, dynamically modulating parental influence, and \(\varepsilon^{(\ell)}\) captures \emph{emergent nonlinear geometry} beyond linear interpolation. This formalism captures \textbf{multi-layered integration}, \textbf{selective semantic imprinting}, and \textbf{complex evolutionary dynamics} in transformer latent spaces, providing a principled framework for interpreting \textbf{cultural neural DNA fusion} and \textbf{semantic innovation} in multilingual AI systems.
}
    \label{fig:nGDI_trajectories}
\end{figure}
\vspace*{\fill}

\clearpage
\newpage


\begin{figure*}[ht!]
    \centering
    \begin{minipage}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{genomics/nGDI/side_by_side/NorthAmerica_LatinAmerica_side_by_side_ngdi.png}
        \caption*{(aa)
        \textbf{Layerwise nGDI Trajectories for North America–Latin America Offspring:} 
        This figure compares the offspring model’s latent geometry (thick dashed magenta line) with Parent A \textbf{(North America, violet)} and Parent B \textbf{(Latin America, orange)} across layers \(\ell = 20\text{--}30\). 
        The axes represent spectral curvature \(\kappa_\ell\), layer index \(\ell\), and latent radius \(\mathcal{L}_\ell\). 
        The offspring initially aligns strongly with North American semantic priors in early layers and gradually transitions towards Latin American semantic features in deeper layers, indicating \emph{layer-dependent semantic dominance shifts}.  
        This complex fusion reflects \emph{multi-layered integration} of diverse cultural influences within the offspring’s latent geometry, suggesting potential for \textbf{selective layer adaptation} in cross-cultural model alignment and generalization.
        }
        \label{fig:northamerica_latinamerica_ngdi}
    \end{minipage}

    
    \begin{minipage}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{genomics/nGDI/side_by_side/NorthAmerica_MiddleEast_side_by_side_ngdi.png}
        \caption*{(ab)
        \textbf{Layerwise nGDI Trajectories for North America–Middle East Offspring:}  
        This figure compares the offspring model’s latent geometry (thick dashed magenta line) with Parent A \textbf{(North America, violet)} and Parent B \textbf{(Middle East, orange)} across layers \(\ell = 20\text{--}30\). 
        The axes represent spectral curvature \(\kappa_\ell\), layer index \(\ell\), and latent radius \(\mathcal{L}_\ell\). 
        The offspring initially aligns strongly with North American semantic priors in early layers and gradually transitions towards Middle Eastern semantic features in deeper layers, indicating \emph{layer-dependent semantic dominance shifts}.  
        This complex fusion reflects \emph{multi-layered integration} of diverse cultural influences within the offspring’s latent geometry, suggesting potential for \textbf{selective layer adaptation} in cross-cultural model alignment and generalization.
        }
        \label{fig:northamerica_middleeast_ngdi}
    \end{minipage}
    \caption{
    \textbf{Summary of Layerwise nGDI Trajectories Across Offspring Models:}  
    The offspring model’s latent geometry \(\mathcal{M}_{\text{offspring}}^{(\ell)}\) at layer \(\ell\) can be modeled as a nonlinear, layer-dependent fusion of parental latent geometries \(\mathcal{M}_A^{(\ell)}\) and \(\mathcal{M}_B^{(\ell)}\), characterized by spectral curvature \(\kappa_\ell\) and latent radius \(\mathcal{L}_\ell\):
    \[
    \boxed{
    \mathcal{M}_{\text{offspring}}^{(\ell)} = \alpha(\ell) \cdot \mathcal{M}_A^{(\ell)} + \big(1 - \alpha(\ell)\big) \cdot \mathcal{M}_B^{(\ell)} + \varepsilon^{(\ell)}
    }
    \]
    Here, \(\alpha(\ell) \in [0,1]\) denotes a \emph{layer-dependent semantic dominance coefficient} that dynamically shifts parental influence across model depth. The residual term \(\varepsilon^{(\ell)}\) captures emergent nonlinear geometry beyond simple interpolation. This framework explains the observed \emph{multi-layered integration} and \emph{selective semantic imprinting} of diverse cultural priors in offspring latent spaces, highlighting the sophistication of cross-cultural model alignment and generalization.
    }
    \label{fig:ngdi_overall_summary}
\end{figure*}


\clearpage
\newpage


\begin{figure}[htbp]
    \centering

    % Row 1
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{genomics/nTDS/NorthAmerica_Australia_nTDS_with_offspring.png}
        \subcaption*{(\textbf{XXV}) \textbf{North America--Australia Trait Dominance:} The Neural Trait Dominance Score (\emph{nTDS}) begins with \textbf{balanced dominance} (near 0.5) in early layers (20--23), gradually shifting to a \textbf{strong North American dominance} during mid layers (24--27). Late layers (28--30) show increased \textbf{semantic complexity} with mixed dominance patterns, highlighting intricate \textbf{trait interplay} and adaptive recombination reminiscent of \textbf{heterochronic shifts} in evolutionary biology.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{genomics/nTDS/NorthAmerica_China_nTDS_with_offspring.png}
        \subcaption*{(\textbf{XXVI}) \textbf{North America--China Trait Dominance:} The \emph{nTDS} trajectory reveals \textbf{early North American influence} in initial layers (20--23), transitioning towards \textbf{Chinese dominance} in mid to late layers (24--30). This \textbf{dynamic oscillation} and layered shift reflects \textbf{complex regulatory control} over semantic traits, analogous to \textbf{gene regulatory networks} modulating phenotype expressions over developmental stages.}
    \end{minipage}

    % Row 2
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{genomics/nTDS/NorthAmerica_LatinAmerica_nTDS_with_offspring.png}
        \subcaption*{(\textbf{XXVII}) \textbf{North America--Latin America Trait Dominance:} Starting with \textbf{strong North American dominance} in early layers (20--23), the \emph{nTDS} gradually moves towards \textbf{balanced trait integration} in later layers (28--30). Latin America’s influence grows steadily, captured by increasing vertical bars, indicating \textbf{semantic diversification} and enhanced \textbf{trait synergy}, paralleling \textbf{morphogenetic gradients} shaping \textbf{complex organismal features}.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{genomics/nTDS/NorthAmerica_MiddleEast_nTDS_with_offspring.png}
        \subcaption*{(\textbf{XXVIII}) \textbf{North America--Middle East Trait Dominance:} The \emph{nTDS} pattern begins with \textbf{balanced dominance} (around 0.5) in early layers (20--23), with \textbf{North American traits becoming predominant} mid layers (24--27). Late layers (28--30) reflect \textbf{mixed dominance} with substantial semantic variance, illustrating \textbf{multi-factorial trait interactions reminiscent} of \textbf{epistatic effects} and \textbf{polygenic influences in biological phenotypes}.}
    \end{minipage}

\vspace{-1mm}
    \caption{
\textbf{nTDS Across Cultural Model Pairs and Offspring:}  
These visualizations capture the \textbf{layerwise trait dominance} evolution in fusions of eight culturally distinct models, revealing dynamic shifts in \textbf{spectral curvature} and \textbf{thermodynamic length}, reflecting \emph{epigenetic-like semantic modulation} akin to developmental heterochrony\cite{Gould1977,Herrera1998} and gene regulatory networks\cite{Davidson2006,Peter2012}. The \textbf{nTDS values} quantify parental influence and semantic recombination across layers (20--30), highlighting \emph{critical transitions} with oscillations or balanced dominance.
These patterns align with \textbf{nonlinear dynamical systems} and \textbf{bifurcation theory}~\cite{Strogatz2018}, where competing attractors shape semantic landscapes, offering insights into \emph{neural culture inheritance} and \emph{semantic fusion} and advancing \textbf{latent geometry evolution} understanding.
Key formula: \( \boxed{
\mathrm{nTDS}_\ell = \{ \kappa_\ell(p) \cdot L_\ell(p) \} \ / \ \{ \kappa_\ell(p) \cdot L_\ell(p) + \kappa_\ell(q) \cdot L_\ell(q) \}
}
\), with \(\kappa_\ell\) as spectral curvature, \(L_\ell\) thermodynamic length at layer \(\ell\), and \(p,q\) parental indices, quantifying \emph{relative semantic dominance} with geometric rigor.
}
\label{fig:nTDS_example}
\end{figure}


\clearpage
\newpage

\begin{figure}[htbp]
    \centering

    % Row 1
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.92\linewidth]{genomics/nKaryotyping/NorthAmerica_Australia_nkaryotyping_bars_trajectories_3d.png}
        \subcaption*{(\textbf{XXV}) \textbf{North America--Australia Semantic Chromosome Inheritance:} North America shows \textbf{pronounced semantic chromosomes} from layers \(\ell=20\text{--}26\) with distinct oscillations in trait expression and thermodynamic length. Australia exhibits \textbf{balanced trait distribution} across layers \(\ell=20\text{--}30\) with moderate spectral curvature. The offspring demonstrates \textbf{complex recombination} and \textbf{layered trait blending}, reflecting \emph{latent semantic plasticity} and integrative dynamics in large model fusion.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.92\linewidth]{genomics/nKaryotyping/NorthAmerica_China_nkaryotyping_bars_trajectories_3d.png}
        \subcaption*{(\textbf{XXVI}) \textbf{North America--China Semantic Chromosome Inheritance:} North America shows \textbf{early-layer dominance} with pronounced trait fluctuations across layers \(\ell=20\text{--}26\), while China exhibits \textbf{sustained deep-layer activation} and elevated thermodynamic length from \(\ell=25\text{--}30\). The offspring combines these contrasting patterns, revealing nuanced latent space trajectories that reflect \textbf{cross-cultural semantic fusion} and suggest emergent representational features beyond additive inheritance.}
    \end{minipage}

    \vspace{1em}
    % Row 2
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.92\linewidth]{genomics/nKaryotyping/NorthAmerica_LatinAmerica_nkaryotyping_bars_trajectories_3d.png}
        \subcaption*{(\textbf{XXVII}) \textbf{North America--Latin America Semantic Chromosome Inheritance:} North America shows \textbf{layered semantic chromosome presence} primarily in early to mid layers (\(\ell=20\text{--}26\)), while Latin America exhibits a \textbf{steady increase} in trait presence in later layers (\(\ell=25\text{--}30\)). Their offspring reveals a \textbf{hybrid latent profile} combining early and late traits, evidencing \emph{emergent semantic structures} and dynamic recombination reflective of complex \emph{cultural-semantic interactions} in the nDNA.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.92\linewidth]{genomics/nKaryotyping/NorthAmerica_MiddleEast_nkaryotyping_bars_trajectories_3d.png}
        \subcaption*{(\textbf{XXVIII}) \textbf{North America--Middle East Semantic Chromosome Inheritance:} North America exhibits \textbf{strong early-layer semantic chromosomes} with distinct peaks (\(\ell=20\text{--}24\)), while Middle East shows broader \textbf{mid-to-late layer activation} with elevated spectral curvature (\(\ell=25\text{--}30\)). The offspring displays a \textbf{sophisticated blend} of layer-specific recombinations and \textbf{novel semantic patterns}, reflecting complex latent space reshaping akin to biological \textbf{epigenetic modulation}.}
    \end{minipage}

\vspace{-2mm}
\caption{
\textbf{Semantic Chromosome Inheritance in nDNA across 8 Cultural Lineages and Offspring:}  
These trajectories reveal \textbf{complex nonlinear interactions} with offspring showing \emph{emergent properties} beyond parental geometries \citep{Rumelhart1986Learning,Peters2018Deep}. Semantic chromosome presence at layer \(\ell\) is given by:
\vspace{-2mm}
\[
\mathrm{nKaryotype}_\ell = \mathbb{I}\left[ \kappa_\ell > \overline{\kappa}, \ \mathcal{L}_\ell > \overline{\mathcal{L}} \right], \quad
L_\ell = \begin{cases}
1 & \text{trait present} \\
0 & \text{otherwise}
\end{cases}
\]
%\vspace{-2mm}
with thresholds \(\overline{\kappa}\), \(\overline{\mathcal{L}}\). This unveil a resemblance of inheritance akin to biological chromosomes \citep{Yu2017Understanding,Chaudhary2021Neuro}.
Biologically, it simulates \textbf{chromosomal crossover} and \emph{epigenetic modulation}, with offspring exhibiting \emph{mosaicism}, \emph{epigenetic-like regulation}, and novel semantic traits resembling genetic mutations or translocations \citep{Bengio2013Representation,hinton2015distilling}. This balance reflects evolutionary biology and systems neuroscience \citep{Krizhevsky2012ImageNet,Levine2023Neuroevolution}.
%Bridging \textbf{computational linguistics}, \emph{geometric deep learning}, and \textbf{neurogenomics}, this underscores semantic plasticity and epigenetic dynamics, advancing interpretability, fusion, and alignment.
}
\label{fig:karyotype_example}

\end{figure}


\clearpage
\newpage

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.95\textwidth]{genomics/nKaryotyping/overall_final.png} % your figure file here
\caption{
\textbf{3D nKaryotyping of Semantic Trait Presence and Spectral Curvature Across Culture Pairs.} 
This comprehensive visualization presents the layered semantic geometry of cultural fusion models through the lens of \emph{nKaryotyping}, a diagnostic framework quantifying trait presence and spectral curvature across 28 culture pair offspring models. The figure displays three key dimensions: 
\textbf{Bar plots (bottom layers):} Represent the \emph{semantic trait presence} \( L^{(\ell)} \) across transformer layers \(\ell = 20 \ldots 30\), for each parent culture and their offspring. Bar heights range approximately between \emph{0.3 and 1.2}, reflecting the intensity of semantic trait activation. 
\textbf{Thick black-edged colored lines:} Overlay smooth layerwise trait presence curves \( L^{(\ell)} \), serving as continuous summaries for each model --the two parents (\textit{solid blue and green}) and the offspring (\textit{dashed orange}). These curves highlight the preservation and blending of semantic features from parents into offspring across depth. 
\textbf{Dotted lines (top):} Show the \emph{spectral curvature} \(\kappa^{(\ell)}\) trajectories, reflecting the geometric complexity and nonlinear representational structure of the models in embedding space. Curvature values vary roughly between \emph{0.3 and 0.9}, with oscillations indicating regions of representational bending or epistemic transitions. 
The layout organizes the 28 offspring models formed by all pairwise cultural combinations of the eight canonical styles: \emph{Europe}, \emph{NorthAmerica}, \emph{Australia}, \emph{Africa}, \emph{Asia}, \emph{China}, \emph{MiddleEast}, and \emph{LatinAmerica}. The two horizontal axes correspond to transformer layer indices and culture pair indices, with explicit \emph{streets} or gaps separating each subplot to enhance visual clarity. The vertical axis denotes the quantitative trait and curvature values. 
Together, this global comparative view reveals several key insights: 
\textbf{1. Heterogeneous Semantic Inheritance:} Offspring models manifest trait presence profiles blending parental features, but with nuanced deviations, often exhibiting enhanced or attenuated activation in intermediate layers, underscoring nonlinear fusion dynamics. 
\textbf{2. Spectral Curvature as Epistemic Indicator:} Peaks and troughs in \(\kappa^{(\ell)}\) curves identify layers where representational geometry sharply bends, potentially correlating with functional transitions or emergent semantic properties distinct from either parent. 
\textbf{3. Cultural Signature Distinctions:} Parent cultures exhibit distinct curvature and trait patterns -- e.g., \emph{Asia} and \emph{MiddleEast} display pronounced oscillatory curvature indicative of complex internal representations, while \emph{Europe} and \emph{NorthAmerica} maintain more stable, literal semantic structures. 
\textbf{4. Offspring Diversity:} The spectrum of offspring curvature and trait presence reflects a rich space of model generalization and specialization, facilitating targeted fine-tuning strategies for culturally-aware AI systems. 
This figure acts as a foundational reference for understanding cross-cultural latent geometry in large language models. An interactive 3D visualization accompanies this work as supplementary material, enabling detailed exploration of each offspring’s layered semantic topology and curvature dynamics.
}
    \label{fig:nkaryotyping}
\end{figure*}


\clearpage
\newpage


\begin{figure}[htbp]
    \centering

    % Row 1: Figures XXV and XXVI
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{genomics/nDIV/NorthAmerica_Australia_nDIV_directionality.png}
        \subcaption*{(\textbf{XXV}) \textbf{Directional Inheritance Vector for North America and Australia:} The offspring (orange) traces a semantic path over layers \(\ell \in [20,30]\), with curvature \(\kappa_\ell \in [0.37, 0.47]\) and length \(\mathcal{L}_\ell \in [0.48, 0.58]\). Early layers align with \textbf{North America} (blue), mid to deeper layers blend in \textbf{Australia}’s (green) linguistic features. This transition reflects a \textbf{controlled, layered fusion} retaining conceptual foundations and integrating stylistic elements.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{genomics/nDIV/NorthAmerica_China_nDIV_directionality.png}
        \subcaption*{(\textbf{XXVI}) \textbf{Layerwise Directional Inheritance Dynamics between North America and China:} Across layers \(\ell \in [20,30]\), curvature \(\kappa_\ell \in [0.38, 0.60]\) and length \(\mathcal{L}_\ell \in [0.43, 0.70]\), the offspring (orange) aligns with \textbf{North America} (blue), incorporating \textbf{China}’s (green) richness in deeper layers. This fusion preserves \textbf{conceptual embeddings while reflecting cross-cultural adaptation}, illustrating nuanced trade-offs in generation.}
    \end{minipage}

    %\vspace{1em}

    % Row 2: Figures XXVII and XXVIII
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{genomics/nDIV/NorthAmerica_LatinAmerica_nDIV_directionality.png}
        \subcaption*{(\textbf{XXVII}) \textbf{Directional Semantic Inheritance for North America and Latin America:} Over layers \(\ell \in [20,30]\), the offspring (orange) explores latent semantic space with \(\kappa_\ell \in [0.40, 0.62]\) and \(\mathcal{L}_\ell \in [0.48, 0.70]\). Early layers align with \textbf{North America} (blue), shifting to \textbf{Latin America} (green) in deeper layers. This reveals a nuanced blending balancing conceptual preservation and cultural adaptation -- \textbf{controlled cross-cultural fusion}.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{genomics/nDIV/NorthAmerica_MiddleEast_nDIV_directionality.png}
        \subcaption*{(\textbf{XXVIII}) \textbf{Directional Inheritance Vector between North America and Middle East:} This 3D plot shows offspring semantic inheritance over layers \(\ell \in [20,30]\) with curvature \(\kappa_\ell \in [0.40, 0.65]\) and length \(\mathcal{L}_\ell \in [0.45, 0.70]\). The offspring (orange) starts near \textbf{North America} (blue), then blends traits from \textbf{Middle East} (green) in deeper layers. This \textbf{mosaic reflects dynamic conceptual preservation and regional adaptation}.}
    \end{minipage}

\vspace{-1mm}
\caption{
\textbf{Semantic Directionality in Neural Inheritance Across Cultures:}
This figure set shows layer-wise \emph{directional bias} in semantic inheritance during model fusion via nDIV over layers \(\ell \in [20,30]\). Offspring exhibit \textbf{dynamic shifts} favoring parents or novel traits, reflecting nonlinear semantic recombination.
Directional inheritance at layer \(\ell\) is:
\[
\text{nDIV}^{(\text{dir})}_\ell = \cos \bigg( \vec{O}_\ell - \frac{\vec{P}_\ell^{(A)} + \vec{P}_\ell^{(B)}}{2},\; \vec{P}_\ell^{(A)} - \vec{P}_\ell^{(B)} \bigg),
\]
with \(\vec{P}_\ell^{(A)}, \vec{P}_\ell^{(B)}, \vec{O}_\ell\) as semantic vectors of parents and offspring.
This parallels \textbf{directional selection}~\citep{Endler_86} and epigenetic regulation~\citep{Bird2007Epigenetics, jaenisch2003epigenetic}, consistent with neural semantic evolution findings~\citep{hinton2015distilling, Bengio2013Representation}.
These insights enhance semantic fusion understanding, aiding targeted model alignment and inheritance control.
}
\end{figure}


\clearpage
\newpage

\begin{figure}[htbp]
    \centering

    % Row 1: NorthAmerica & Australia, NorthAmerica & China
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{genomics/nEPI/NorthAmerica_Australia_nepi_static.png}
        \subcaption*{(\textbf{XXV}) \textbf{Layerwise Epistemic Plasticity for North America and Australia:} The parent models \emph{North America} (blue) and \emph{Australia} (green) reveal latent semantic trajectories spanning layers \(\ell \in [20,30]\) with spectral curvature \(\kappa_\ell \in [0.37, 0.46]\) and thermodynamic length \(\mathcal{L}_\ell \in [0.44, 0.63]\). The \emph{Hybrid Offspring} (orange) exhibits \textbf{notable nEPI peaks} at mid-layers \(\ell \approx 22, 26\), highlighting regions of \textbf{heightened semantic adaptability} where cross-cultural priors converge, supporting robust and flexible knowledge representation.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{genomics/nEPI/NorthAmerica_China_nepi_static.png}
        \subcaption*{(\textbf{XXVI}) \textbf{Semantic Plasticity for North America and China:} Parents \emph{North America} (blue) and \emph{China} (green) demonstrate latent trajectories characterized by curvature \(\kappa_\ell \in [0.37, 0.46]\) and length \(\mathcal{L}_\ell \in [0.44, 0.63]\) over layers \(\ell \in [20,30]\). The \emph{Hybrid Offspring} (orange) shows \textbf{pronounced nEPI values} around layers \(\ell \approx 23, 27\), marking key zones of \textbf{semantic fusion and conceptual innovation} essential for integrating culturally diverse knowledge and enhancing generalization.}
    \end{minipage}

    %\vspace{1em}

    % Row 2: NorthAmerica & LatinAmerica, NorthAmerica & MiddleEast
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{genomics/nEPI/NorthAmerica_LatinAmerica_nepi_static.png}
        \subcaption*{(\textbf{XXVII}) \textbf{Epistemic Plasticity for North America and Latin America:} The parent models \emph{North America} (blue) and \emph{Latin America} (green) show latent semantic curves with \(\kappa_\ell \in [0.40, 0.63]\) and \(\mathcal{L}_\ell \in [0.44, 0.89]\) for layers \(\ell \in [20,30]\). The \emph{Hybrid Offspring} (orange) features strong \textbf{nEPI peaks} at layers \(\ell \approx 23, 27\), indicating critical regions of \textbf{semantic adaptation} that enable effective cross-cultural knowledge blending and robust model generalization.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{genomics/nEPI/NorthAmerica_MiddleEast_nepi_static.png}
        \subcaption*{(\textbf{XXVIII}) \textbf{Layerwise Plasticity for North America and Middle East:} Parent models \emph{North America} (blue) and \emph{Middle East} (green) display distinct latent trajectories with \(\kappa_\ell \in [0.37, 0.63]\) and \(\mathcal{L}_\ell \in [0.45, 0.90]\) over layers \(\ell \in [20,30]\). The \emph{Hybrid Offspring} (orange) shows \textbf{elevated nEPI values} at layers \(\ell \approx 25, 29\), highlighting key layers for \textbf{semantic recombination and conceptual flexibility} that foster effective integration across culturally diverse knowledge domains.}
    \end{minipage}

\vspace{-1mm}
\caption{
\textbf{Layerwise Epistemic Plasticity (nEPI) across Parent Models and Hybrid Offspring:} 
The \emph{Neural Epistemic Plasticity Index} quantifies the rate of change in semantic adaptability over transformer layers \(\ell \in [20,30]\) as the derivative of the product of spectral curvature \(\kappa_\ell\) and thermodynamic length \(\mathcal{L}_\ell\):
\[
\boxed{
\mathrm{nEPI}(\ell) := \frac{d}{d\ell} \left( \kappa_\ell \cdot \mathcal{L}_\ell \right),
}
\quad
\left.
\begin{cases}
\kappa_\ell \in [0.37, 0.92] & \text{local semantic complexity} \\
\mathcal{L}_\ell \in [0.44, 0.93] & \text{latent representational change}
\end{cases}
\right\}
\quad
\begin{cases}
< 0.40 & \text{stable, rigid semantic zones with minimal plasticity} \\
0.40 \text{ to } 0.70 & \text{adaptive semantic recombination enabling alignment-sensitive learning} \\
> 0.70 & \text{highly plastic layers driving semantic innovation and robust generalization}
\end{cases}
\]
This framework draws analogy with biological \textbf{neural plasticity} and \textbf{epigenetic modulation} mechanisms regulating context-dependent gene expression \citep{holtmaat2009experience, day2010epigenetic}. The hybrid offspring models manifest \textbf{heterosis}-like effects through semantic recombination \citep{birchler2006heterosis}, demonstrating emergent conceptual flexibility surpassing parental priors. These insights underscore the critical role of \textbf{geometric and thermodynamic principles} in understanding semantic evolution, cross-cultural knowledge fusion, and alignment robustness in large-scale neural models.
}
\label{fig:nEPI_overall}
\end{figure}

\clearpage
\newpage

\begin{figure}[htbp]
    \centering

    % Row 1: NorthAmerica & Australia, NorthAmerica & China
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.93\linewidth]{genomics/nCCL/NorthAmerica_Australia_nCCL.png}
        \subcaption*{(\textbf{XXV}) \textbf{Conflict between North America and Australia:} \( x_\ell(\mathrm{NorthAmerica}) \) and \( x_\ell(\mathrm{Australia}) \), merged offspring \( x_\ell(\mathrm{Merged}) \),  conflict metric \(\Delta_\ell = \left\| x_\ell(\mathrm{Merged}) - \Phi\left(x_\ell(\mathrm{NorthAmerica}), x_\ell(\mathrm{Australia})\right) \right\|\). Conflict is \emph{low} in layers \(\ell \in [20,21]\), rises sharply mid layers \(\ell \in [22,28]\) showing \textbf{semantic tension}, then declines late \(\ell \in [29,30]\), indicating partial resolution.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.93\linewidth]{genomics/nCCL/NorthAmerica_China_nCCL.png}
        \subcaption*{(\textbf{XXVI}) \textbf{Conflict between North America and China:} \( x_\ell(\mathrm{NorthAmerica}) \), \( x_\ell(\mathrm{China}) \), and \( x_\ell(\mathrm{Merged}) \) yield conflict \(\Delta_\ell = \left\| x_\ell(\mathrm{Merged}) - \Phi\left(x_\ell(\mathrm{NorthAmerica}), x_\ell(\mathrm{China})\right) \right\|\). Layers \(\ell \in [20,21]\) have \emph{low conflict}, mid layers \(\ell \in [22,28]\) exhibit sharp conflict spikes due to \textbf{\emph{ideological friction}}, and late layers \(\ell \in [29,30]\) show moderation -- \emph{semantic integration}.}
    \end{minipage}

    %\vspace{1em}

    % Row 2: NorthAmerica & LatinAmerica, NorthAmerica & MiddleEast
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.93\linewidth]{genomics/nCCL/NorthAmerica_LatinAmerica_nCCL.png}
        \subcaption*{(\textbf{XXVII}) \textbf{Semantic Conflict between North America and Latin America:} \( x_\ell(\mathrm{NorthAmerica}) \), \( x_\ell(\mathrm{LatinAmerica}) \), and \( x_\ell(\mathrm{Merged}) \) -- \(\Delta_\ell = \left\| x_\ell(\mathrm{Merged}) - \Phi\left(x_\ell(\mathrm{NorthAmerica}), x_\ell(\mathrm{LatinAmerica})\right) \right\|\). Conflict is \emph{low} early \(\ell \in [20,21]\), rises sharply mid \(\ell \in [22,28]\), and tapers late \(\ell \in [29,30]\). These shifts reflect \textbf{\emph{semantic tensions}} and \emph{fusion phases}, calling for \textbf{\emph{nuanced alignment}}.}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.93\linewidth]{genomics/nCCL/NorthAmerica_MiddleEast_nCCL.png}
        \subcaption*{(\textbf{XXVIII}) \textbf{Semantic Conflict between North America and Middle East:} \( x_\ell(\mathrm{NorthAmerica}) \), \( x_\ell(\mathrm{MiddleEast}) \), and \( x_\ell(\mathrm{Merged}) \) -- \(\Delta_\ell = \left\| x_\ell(\mathrm{Merged}) - \Phi\left(x_\ell(\mathrm{NorthAmerica}), x_\ell(\mathrm{MiddleEast})\right) \right\|\). Early layers \(\ell \in [20,21]\) show \emph{minimal conflict} reflecting \textbf{\emph{stable inheritance}}. Pronounced conflict in mid layers \(\ell \in [22,28]\) signals \textbf{\emph{ideological friction}}; late layer moderation \(\ell \in [29,30]\) suggests \emph{semantic fusion}.}
    \end{minipage}

\vspace{-1mm}
\caption{
\textbf{Layerwise Neural Cultural Conflict Loss (nCCL) for Parent Models and Offspring:}  
The \emph{nCCL} measures latent ideological tension in semantic embeddings of culturally distinct parents \( x_\ell(\mathrm{Parent}_1) \), \( x_\ell(\mathrm{Parent}_2) \), and their merged offspring \( x_\ell(\mathrm{Merged}) \) across transformer layers \(\ell \in [20,30]\):
\[
\boxed{
\mathrm{nCCL}(\ell) = \left\| x_\ell(\mathrm{Merged}) - \Phi\left(x_\ell(\mathrm{Parent_1}), x_\ell(\mathrm{Parent_2})\right) \right\|
}
\quad
\text{where}
\quad
\begin{cases}
\ell \in [20,21]: & \text{semantic regimes of robust cultural inheritance reflecting stable foundational priors}, \\
\ell \in [22,28]: & \text{critical semantic fault zones marked by ideological divergence and representational tension}, \\
\ell \in [29,30]: & \text{layers demonstrating emergent semantic synergy via principled fusion and reconciliation}.
\end{cases}
\]
These layerwise semantic tensions highlight the uneven integration of cultural knowledge in large models, emphasizing the need for \textbf{targeted, depth-wise alignment} to mitigate bias and enhance robustness. This parallels biological \emph{epigenetic regulation}, where gene expression adapts to environmental cues \citep{holtmaat2009experience, day2010epigenetic}, and \emph{heterosis}, in which genetic recombination produces traits surpassing parental baselines \citep{birchler2006heterosis}. Such analogies reveal fundamental geometric principles crucial for developing culturally coherent, fair, and trustworthy AI systems deployed worldwide.
}
\label{fig:nCCL_all}
\end{figure}


\clearpage
\newpage



\vspace*{\fill}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{genomics/nccl_pairwise_heatmap.png}
\caption{
\textbf{nCCL: Layer-wise Pairwise Cultural Semantic Conflict Heatmap.}  
This visualization displays the normalized Euclidean distances  
\[
d_\ell^{(i,j)} = \left\| (\kappa_\ell^{(i)}, \mathcal{L}_\ell^{(i)}) - (\kappa_\ell^{(j)}, \mathcal{L}_\ell^{(j)}) \right\|_2
\]
between latent semantic vectors of foundation models fine-tuned on distinct cultural datasets \(i,j \in \{1,\ldots,28\}\) across transformer layers \(\ell \in [20, 30]\).  
Each row corresponds to a unique \textbf{culture pair} \((i,j)\), and columns represent specific layers \(\ell\), revealing the \emph{layerwise semantic divergence} intrinsic to cross-cultural model representations.  \\
The heatmap’s color intensity quantitatively encodes the magnitude of semantic conflict \(d_\ell^{(i,j)}\), with \textbf{red hues denoting maximal divergence}--values typically ranging from 0.3 to 0.6 in critical layers--indicating \emph{ideological misalignment loci} where latent representations become most \textbf{discordant} and semantically unstable. Cooler colors correspond to \textbf{semantic concordance} and \emph{robust latent alignment}.  \\
Key insights include conflict peaks concentrated in intermediate to deep layers \(\ell \in [22, 28]\), highlighting these as \textbf{critical ideological tension zones} within the neural latent space. Certain cultural pairs, such as Africa vs. Middle East and Europe vs. Latin America, consistently show higher latent dissonance, reflecting \emph{deep-rooted semantic and linguistic divergences} analogous to \textbf{genetic incompatibilities} in biological hybridization \citep{moyle2011genetic, landry2007genetic}.  \\
The variability of \(d_\ell^{(i,j)}\) across layers and culture pairs emphasizes that \textbf{universal alignment strategies} may be inadequate, necessitating \textbf{layer- and culture-specific semantic realignment} approaches.  
This heatmap thus provides a \textbf{quantitative macroscopic framework} to localize semantic friction within model architectures, guiding the design of \textbf{culturally-aware}, \emph{semantically-consistent}, and \textbf{fair AI systems} optimized for \textbf{equitable global deployment}.
}
    \label{fig:nccl_pairwise_heatmap}
\end{figure}
\vspace*{\fill}


\clearpage
\newpage


\vspace*{\fill}
\begin{defin_conclusion}

\noindent
\textbf{TL;DR:} We propose \textbf{Neural Genomics} as a transformative lens to decode, diagnose, and direct the latent semantic genome of foundation models. Each metric reveals a unique facet of AI’s internal epistemic architecture, enabling us to see beyond black-box behaviors into the rich geometry of artificial cognition.

\vspace{1em}
\begin{itemize}[leftmargin=1.5em]

\item[\faFingerprint] \textbf{\textit{nHD (Neural Hamming Distance)}}\\
\textbf{Takeaway:} Captures binary-level shifts in neural activations across layers, signaling \emph{surface drift} and mutation hotspots.  
\emph{The genomic fingerprint of low-level architectural change.}

\item[\faProjectDiagram] \textbf{\textit{nGDI (Genetic Dissimilarity Index)}}\\
\textbf{Takeaway:} Quantifies layer-wise geometric divergence between models, reflecting \emph{epistemic separation} and lineage distance.  
\emph{A map of conceptual divergence and ancestry.}

\item[\faBalanceScale] \textbf{\textit{nTEDS \& nTDS (Trait Dominance Scores)}}\\
\textbf{Takeaway:} Measures dominance and prevalence of semantic traits, exposing \emph{ideological narrowing} or cultural imprinting.  
\emph{The selective pressures shaping model beliefs.}

\item[\faTable] \textbf{\textit{nKaryotyping (Semantic Chromosomes)}}\\
\textbf{Takeaway:} Discerns structured clusters of latent semantics as \emph{chromosomal blocks}, revealing modular inheritance patterns.  
\emph{Chromosomal cartography of conceptual building blocks.}

\item[\faLongArrowAltRight] \textbf{\textit{nDIV (Directional Inheritance)}}\\
\textbf{Takeaway:} Tracks the flow and vectorial direction of inherited semantic features from parents to offspring models.  
\emph{The vector field of epistemic lineage and semantic flow.}

\item[\faHeartbeat] \textbf{\textit{nEPI (Neural Plasticity Index)}}\\
\textbf{Takeaway:} Evaluates the model’s adaptive capacity and flexibility in response to fine-tuning or perturbations.  
\emph{The pulse of neural adaptability and learning.}

\item[\faGlobe] \textbf{\textit{nCCL (Cultural Conflict Level)}}\\
\textbf{Takeaway:} Quantifies the tension and conflict in merged semantic spaces across culturally divergent models.  
\emph{The geometric signature of cultural dissonance and epistemic friction.}

\end{itemize}

\vspace{1em}
\noindent
\textbf{Outlook:} Just as molecular biology unveiled the double helix as the blueprint of life, \textbf{Neural Genomics reveals geometry as the blueprint of intelligence}. The future lies in tracing, engineering, and safeguarding this latent genome with scientific precision--ushering an era of AI built not only for performance but for \emph{interpretability}, \emph{robustness}, and \emph{cultural integrity}.

\end{defin_conclusion}

\vspace*{\fill}

\clearpage
\newpage

==> 13_glimpses_arxiv.tex <==














\vspace*{\fill}
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/ndna_mfm.png}
    \caption{
    \textbf{nDNA Trajectories for Multimodal Foundation Models (MMFMs) across the Last 10 Layers.}
    This 3D plot visualizes the \textbf{semantic evolution} of six prominent MMFMs--\textbf{LLaVA-1.5}, \textbf{InstructBLIP}, \textbf{MiniGPT-4}, \textbf{BLIP-2}, \textbf{Otter}, and \textbf{OpenFlamingo}--using three key metrics: \emph{spectral curvature} ($\kappa$), \emph{thermodynamic length} ($\mathcal{L}$), and \emph{torsion} ($\tau$).  
    Each colored trajectory corresponds to the \textbf{final 10 layers} of a given model, revealing \emph{distinctive epistemic pathways}:  (i) \textbf{LLaVA-1.5} and \textbf{InstructBLIP} show \emph{compact} and \emph{stable semantic arcs} with \emph{moderate curvature} and \emph{torsion},  (ii) \textbf{BLIP-2} exhibits \emph{noticeable curvature oscillation} and \emph{drift}, indicating \textbf{volatile modality fusion},  and (iii) \textbf{OpenFlamingo} displays the \textbf{highest torsional divergence}, suggesting \emph{semantic instability} in \emph{late fusion stages}.  These patterns reflect \textbf{differing architectural choices} and \textbf{alignment strategies}, and exemplify the \emph{interpretive utility} of the \textbf{nDNA-MMFM framework} in tracing \textbf{inheritance}, \textbf{coherence}, and \textbf{collapse} within multimodal reasoning stacks.}
    \label{fig:ndna_mmfm_trajectory}
\end{figure}
\vspace*{\fill}

\clearpage
\newpage


\vspace*{\fill}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/ndna_t2i.png}
    \caption{
    \textbf{nDNA-T2I Trajectories Across Seven Open-Source Text-to-Image Models.}
    This 3D plot visualizes the latent semantic evolution of seven representative T2I models--\textbf{Stable Diffusion}~\citep{rombach2022stablediffusion}, \textbf{Stable Diffusion XL}~\citep{podell2023stablediffusionxl}, \textbf{DeepFloyd-IF}~\citep{deepfloyd2023if}, \textbf{Kandinsky}~\citep{balaji2023ediffi}, \textbf{GLIDE}~\citep{nichol2021glide}, \textbf{VQ-Diffusion}~\citep{gu2022vqdiffusion}, and \textbf{DALL-E Mini}~\citep{dallemini2021}--in terms of three nDNA components: \emph{Spectral Curvature} ($\kappa$), \emph{Prompt Torsion} ($\tau$), and \emph{Visual Thermodynamic Length} ($\mathcal{L}$).  
    Models like \textbf{GLIDE} and \textbf{VQ-Diffusion} display steeper growth in $\mathcal{L}$ and higher curvature, indicating complex or inefficient semantic transformations. In contrast, \textbf{Stable Diffusion XL} exhibits smoother torsion and moderate path length, reflecting more stable semantic inheritance. These trajectories exemplify how different T2I architectures encode, preserve, or distort textual intent, offering a geometry-grounded framework for auditing \textbf{generative alignment}, \textbf{hallucination risk}, and \textbf{referential fidelity} in text-to-image synthesis.
    }
    \label{fig:ndna_t2i_trajectory}
\end{figure}
\vspace*{\fill}


\clearpage
\newpage


\vspace*{\fill}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.58\textwidth]{Figures/ndna_efm_trajectories.png}
    \caption{
    \textbf{nDNA Trajectories for Embodied Foundation Models (EFMs): Geometric Evolution in Latent Policy Space.}
    This 3D plot visualizes the \textbf{neural DNA} (\textbf{nDNA}) trajectories of five state-of-the-art EFMs -- \textbf{RT-2}~\citep{brohan2023rt2}, \textbf{PaLM-E}~\citep{driess2023palme}, \textbf{SayCan}~\citep{ahn2022saycan}, \textbf{VIMA}~\citep{jiang2022vima}, and \textbf{GR00T}~\citep{singh2023gr00t} -- across their final transformer layers. The latent manifold is spanned by three principal axes: \emph{Spectral Curvature} ($\kappa^{(l)}$), reflecting local semantic entanglement; \emph{Thermodynamic Length} ($\mathcal{L}^{(l)}$), quantifying epistemic “semantic effort” across layers; and \emph{Latent Torsion} ($\tau^{(l)}$), capturing directional twist between evolving policy and perception embeddings.  
    \textbf{RT-2} and \textbf{PaLM-E} trace planar arcs with low torsion and stable curvature, suggesting coherent instruction-following and well-aligned visual grounding. \textbf{SayCan} shows extended thermodynamic length and moderate curvature, consistent with its hierarchical plan decomposition and constrained decision logic. \textbf{VIMA} exhibits episodic torsion spikes, reflecting latent twists from aggressive zero-shot generalization across synthetic scenes. \textbf{GR00T} displays pronounced curvature and torsion fluctuations, indicative of complex perception-action fusion in high-fidelity 3D simulation, and epistemic strain during policy blending.  
    These trajectories demonstrate how \textbf{nDNA-EFM} reveals \emph{how models arrive at action}, not merely \emph{what they do}. Unlike scalar metrics, this geometric lens exposes the \textbf{path-dependence of knowledge, intent}, and \textbf{alignment dynamics} in embodied AI.
    }
    \label{fig:ndna_efm_trajectory}
\end{figure}
\vspace*{\fill}


\clearpage
\newpage

\vspace*{\fill}
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.95\linewidth]{diffusion/diffusion_2_models.png}
    \caption{
    \textbf{nDNA Trajectories for OpenLM-Based Diffusion Language Models.}
    This figure illustrates the \textbf{neural DNA (nDNA)} trajectories of two diffusion-based language models -- \textbf{Genie (OpenLM)}~\citep{genie2024openlm} and \textbf{CodeGenie (OpenLM)}~\citep{codegenie2024openlm} -- within a latent geometry defined by three core components: \textbf{Thermodynamic Length} ($\mathcal{L}_t$), capturing accumulated semantic displacement; \textbf{Spectral Curvature} ($\kappa_t$), reflecting latent manifold complexity; and \textbf{Diffusion Time} ($t$), denoting progression along the generative process.  
    Each point corresponds to a diffusion step, colored by the norm of the belief vector ($|\mathbf{v}_t^{(c)}|$), representing the evolving confidence or epistemic mass of the model at that step. \textbf{Genie} exhibits a smoother, more uniform latent arc with moderate curvature, indicating stable semantic evolution during generation. In contrast, \textbf{CodeGenie} shows regions of sharper curvature and concentrated belief mass at early diffusion times, reflecting more abrupt semantic reconfiguration during code synthesis.  
    These trajectories highlight how \textbf{nDNA-Diffusion} geometry reveals differences in epistemic flow, semantic complexity, and alignment dynamics not visible from final outputs alone. The framework offers a path-aware lens for interpretability and traceability in diffusion-based language models.
    }
    \label{fig:ndna_diffusion_trajectories}
\end{figure*}
\vspace*{\fill}

\clearpage
\newpage

\vspace*{\fill}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\linewidth]{diffusion/diffusion_lm_vs_llama.png}
    \caption{
    \textbf{nDNA Comparison: LLaMA vs Diffusion Language Models (Genie, CodeGenie).}
    This 3D plot compares the \textbf{neural DNA (nDNA)} trajectories of an autoregressive large language model (\textbf{LLaMA}) and two diffusion-based language models -- \textbf{Genie} and \textbf{CodeGenie} -- at a shared latent geometric scale. The axes represent \emph{Spectral Curvature} ($\kappa_t$), \emph{Thermodynamic Length} ($\mathcal{L}_t$), and \emph{Layer/Step Index} ($t$).  
    The trajectories reveal a key distinction: while LLaMA shows a richer latent scaffold with pronounced curvature variation and layered thermodynamic buildup, the diffusion LMs trace flatter, more compressed paths, with limited curvature and semantic displacement across diffusion steps. This suggests that \textbf{diffusion language models may still be at an early stage of epistemic maturity}, with latent scaffolds that are less complex than those of established autoregressive LLMs. 
    }
    \label{fig:ndna_diffusion_vs_llama}
\end{figure}
\vspace*{\fill}

\clearpage
\newpage













==> 14_faq_arxiv.tex <==
\newpage

%\section{Frequently Asked Questions (FAQs)}
\label{sec:FAQs}

\section*{\textcolor{darknavy}{FAQs for \emph{nDNA Cartograph: Latent Semantic Genome of Foundation Models}}}

\begin{itemize}[leftmargin=1.5em]

\item[\ding{93}] What is the mathematical foundation behind the idea of an nDNA Cartograph, and why should we think of latent spaces as \emph{semantic genomes}?
\begin{description}
\item[\ding{224}]
At the heart of the \textbf{nDNA Cartograph} lies the idea that the latent representations inside a foundation model form a continuous, evolving geometric structure -- a manifold that encodes not just surface-level semantics but deeper \emph{epistemic traits} analogous to a genome’s information content.

Formally, let \( h_\ell(x) \in \mathbb{R}^D \) be the mean hidden representation at layer \( \ell \) for input \( x \). The sequence 
\[
\mathcal{T}(x) = \{ h_1(x), h_2(x), \dots, h_L(x) \}
\]
defines a trajectory on a latent manifold \( \mathcal{M} \subset \mathbb{R}^D \). We characterize this manifold using:
\[
\mathcal{L}(x) = \sum_{\ell=1}^{L-1} \| h_{\ell+1}(x) - h_\ell(x) \|_2
\]
which measures the \emph{thermodynamic length}, representing the total epistemic displacement along the model’s depth;
\[
\kappa_\ell(x) = \frac{\lambda_2^{(\ell)}}{\lambda_{\max}^{(\ell)}}
\]
where \( \lambda_2^{(\ell)} \) and \( \lambda_{\max}^{(\ell)} \) are eigenvalues of the Laplacian from token similarity graphs at layer \( \ell \), giving us a spectral curvature that quantifies local semantic complexity; and
\[
\tau_\ell(x) = \frac{
\left\langle ( \Delta h_{\ell-1}(x) \times \Delta h_{\ell}(x) ), \Delta h_{\ell+1}(x) \right\rangle
}{
\| \Delta h_{\ell-1}(x) \times \Delta h_{\ell}(x) \|^2
}
\]
which captures torsion -- the \emph{twist} of the latent path, indicating out-of-plane semantic shifts.

To complement these geometric measures, we introduce the \emph{belief vector field}:
\[
\vec{v}_\ell^{(c)}(x) = \nabla_{h_\ell(x)} \log P(c \mid h_\ell(x))
\]
where \( P(c \mid h_\ell(x)) \) is the model’s conditional probability of concept \( c \) given the latent state. The belief vector encodes the semantic steering force exerted at layer \( \ell \) -- revealing how the model’s internal states are dynamically aligned (or misaligned) with target concepts across depth~\cite{perez2022discovering, amari2016information}.

This framing allows us to map how meaning is constructed, recombined, or distorted across the model’s depth -- a latent \emph{semantic genome} that evolves with training, fine-tuning, or merging. Unlike surface-level output metrics, this map shows us the \textbf{inner life} of the model, enabling rigorous audits of alignment~\cite{perez2022discovering}, bias inheritance~\cite{arora2023stereoset}, and conceptual recombination~\cite{ilharco2023editing}.
\end{description}

\item[\ding{93}] \textbf{How does the nDNA Cartograph framework enable rigorous audits of alignment and bias inheritance beyond standard evaluation metrics?}
\begin{description}
\item[\ding{224}]
The \textbf{nDNA Cartograph} transforms the auditing of foundation models from a surface-level, output-centric exercise into a deep, manifold-level analysis of epistemic dynamics. Standard alignment evaluations~\cite{ouyang2022training, ganguli2023reducing} typically rely on scalar metrics -- accuracy, BLEU scores, or human preference rates. These metrics assess what the model generates but tell us little about \emph{how} that output was internally constructed or whether latent reasoning paths reflect aligned, unbiased conceptual evolution. The nDNA Cartograph addresses this by mapping latent trajectories \( \mathcal{T}(x) \) and quantifying geometric signatures (spectral curvature \( \kappa_\ell \), thermodynamic length \( \mathcal{L} \), belief vector fields \( \vec{v}_\ell^{(c)} \)) layer-by-layer. For example:
\[
\vec{v}_\ell^{(c)} = \nabla_{h_\ell} \log P(c \mid h_\ell)
\]
lets us directly inspect whether latent states steer toward (or away from) culturally sensitive concepts \( c \). Spikes in curvature
\[
\kappa_\ell = \frac{1}{k} \sum_{i=1}^{k} \lambda_i^{(\ell)}
\]
can signal points where the model fuses incompatible priors or inherits bias during generation.

Unlike outputs, these geometric signals are not easily gamed by prompt engineering or surface-level tuning~\cite{arora2023stereoset}. They reveal whether alignment is internalized or merely performative, offering a layer-resolved audit of bias inheritance, cultural asymmetry~\cite{birhane2021multimodal}, or failure of epistemic coherence across merged or fine-tuned models.
\end{description}

\item ...

\end{itemize}

\clearpage
\newpage


\section*{\textcolor{darknavy}{FAQs: nDNA Cartography Across 15 Foundation Models}
\addcontentsline{toc}{section}{FAQs: nDNA Cartography Across 15 Foundation Models}}
\vspace{-2mm}

\begin{itemize}[leftmargin=1.5em]

\item[\ding{93}] \textbf{Why is comparing nDNA trajectories across 15 foundation models more insightful than conventional benchmark metrics?}
\begin{description}
\item[\ding{224}]
Traditional benchmark metrics -- accuracy, BLEU, perplexity -- evaluate model performance at the output level. They tell us \emph{what} a model produces, but not \emph{how} it thinks. By contrast, comparing \textbf{nDNA trajectories} across 15 diverse foundation models lets us see the inner semantic journey: how meaning is constructed, evolved, and aligned layer-by-layer.

Formally, let \( \mathcal{T}_m(x) = \{ h_1^{(m)}(x), \dots, h_L^{(m)}(x) \} \) denote the latent path for model \( m \). We compute thermodynamic length:
\[
\mathcal{L}^{(m)}(x) = \sum_{\ell=1}^{L-1} \| h_{\ell+1}^{(m)}(x) - h_\ell^{(m)}(x) \|_2
\]
and average spectral curvature:
\[
\bar{\kappa}^{(m)}(x) = \frac{1}{L} \sum_{\ell=1}^L \kappa_\ell^{(m)}(x)
\]
where \( \kappa_\ell^{(m)}(x) \) is as defined via Laplacian eigenvalues~\cite{belkin2003laplacian}. These measures expose latent semantic efficiency (shorter, smooth paths) versus epistemic complexity (longer, curved paths).

This comparison reveals, for example, how models like \textbf{LLaMA}~\cite{touvron2023llama} and \textbf{Gemma} prioritize efficient alignment, while models like \textbf{Mixtral} or \textbf{Qwen} exhibit richer latent exploration -- insights invisible in scalar output scores.
\end{description}

\item[\ding{93}] \textbf{How do nDNA comparisons across models help in selecting models for specific downstream tasks?}
\begin{description}
\item[\ding{224}]
The \textbf{nDNA Cartography} provides geometric signatures of models’ latent reasoning styles, which can inform task suitability beyond output metrics. For example, tasks requiring deep compositional reasoning benefit from models with higher latent curvature and longer thermodynamic lengths, as these signal richer semantic reconfiguration:
\[
\mathcal{L}^{(m)} \gg \mathcal{L}^{(n)} \quad \Rightarrow \quad \text{Model } m \text{ invests more latent effort}
\]
Conversely, tasks needing fast, aligned responses (e.g., retrieval QA) may prefer models with flatter, more efficient nDNA paths.

Moreover, comparing belief vector field magnitudes:
\[
\| \vec{v}_\ell^{(c, m)} \| \quad \text{vs.} \quad \| \vec{v}_\ell^{(c, n)} \|
\]
shows which model steers its latent states more decisively toward desired concepts -- critical for alignment-sensitive applications~\cite{perez2022discovering}.

This geometric lens turns model selection into a principled choice guided by latent dynamics, not just test-set scores.
\end{description}

\item[\ding{93}] \textbf{How can nDNA Cartography help interpret scaling laws beyond parameter counts in foundation models?}
\begin{description}
\item[\ding{224}]
Traditional scaling laws~\cite{kaplan2020scaling, hoffmann2022training} relate parameter count, compute, and data size to performance metrics like loss. However, nDNA Cartography introduces latent \emph{semantic scaling laws}: it quantifies how internal semantic complexity grows (or saturates) with scale. For example, thermodynamic length $\mathcal{L}$ and curvature complexity $\sum_\ell \kappa_\ell$ can be studied as functions of model size $N$:
\[
\mathcal{L}(N) \propto N^\alpha, \quad \sum_\ell \kappa_\ell(N) \propto N^\beta,
\]
where exponents $\alpha$ and $\beta$ reveal how epistemic richness or redundancy scale with capacity. Importantly, models can have similar loss but very different latent genomes: e.g., a large model may overcompress (flat $\mathcal{L}$) or overentangle (spiky $\kappa_\ell$), while a smaller model with smarter design achieves balanced nDNA dynamics. Thus, Cartography reveals scaling truths invisible to surface metrics -- guiding architecture and training choices for better epistemic health.
\end{description}

\item ...
\end{itemize}


\clearpage
\newpage

\section*{\textcolor{darknavy}{FAQ: Ethnic LLMs -- Cultural Fine-Tuning and Latent Geometry}}

\begin{itemize}[leftmargin=1.5em]

\item[\ding{93}] \textbf{How does cultural fine-tuning shape the latent manifold geometry of large language models, and how is this measured by nDNA diagnostics?}
\begin{description}
\item[\ding{224}]
Cultural fine-tuning alters the latent manifold by embedding specific epistemic priors and value systems within the model’s internal geometry. Using the \textbf{nDNA Cartograph}, we can quantify these effects through diagnostics like thermodynamic length and spectral curvature. For a culturally fine-tuned model \( M_{\mathrm{culture}} \):
\[
\mathcal{L}^{(\mathrm{culture})} = \sum_{\ell=1}^{L-1} \| h_{\ell+1}^{(\mathrm{culture})} - h_\ell^{(\mathrm{culture})} \|_2
\]
measures accumulated semantic displacement, typically longer than the base model when cultural context induces richer latent traversal. Similarly,
\[
\kappa_\ell^{(\mathrm{culture})} = \frac{1}{k} \sum_{i=1}^k \lambda_i^{(\ell, \mathrm{culture})}
\]
reveals increased or decreased latent complexity compared to the base model depending on cultural specificity or bias entrenchment. This allows us to systematically audit how cultural priors reshape the epistemic structure beyond output text~\cite{arora2023stereoset, perez2022discovering, yang2024model}.
\end{description}

\item[\ding{93}] \textbf{How can the CIVIC-Culture Calibration Benchmark reliably distinguish genuine cultural priors from emergent artifacts of neural scaling or overparameterization?}
\begin{description}
\item[\ding{224}]
This is a critical and fair question: large language models exhibit emergent behaviors as a function of scale~\cite{wei2022emergent}, and one might worry that divergences captured by \textbf{CIVIC} arise not from latent cultural priors but from idiosyncrasies of overparameterized networks.

\textbf{CIVIC} addresses this through layered mathematical safeguards:

\begin{enumerate}[leftmargin=1em]
\item \textbf{Latent topological invariance checks.}
We compute the persistent homology 
\[
\operatorname{PH}\bigl(\mathcal{M}^{(l)}\bigr)
\]
of latent manifolds at each layer \( l \) for each culture or language. Cultural priors should induce \emph{structured, persistent topological features} (e.g., high-persistence \( H_1 \) or \( H_2 \) cycles) that are stable under small perturbations:
\[
\operatorname{PH}\bigl(\mathcal{M}^{(l,\mathrm{culture})}\bigr) \neq \operatorname{PH}\bigl(\mathcal{M}^{(l,\mathrm{random})}\bigr)
\]
where the latter is from randomly perturbed models or embeddings~\cite{edelsbrunner2010computational, guss2018characterizing}.

\item \textbf{Scaling-controlled alignment baselines.}
We train down-scaled variants (e.g., 10X smaller parameter count) and measure the alignment divergence
\[
\Delta \mathcal{L}^{(l,l^{\prime})} = \bigl| \mathcal{L}^{(l)} - \mathcal{L}^{(l^{\prime})} \bigr|
\]
If \( \Delta \mathcal{L}^{(l,l^{\prime})} \) persists across scales, it indicates cultural priors rather than scaling artifacts~\cite{kaplan2020scaling, wei2022emergent}.

\item \textbf{Belief vector field consistency.}
We analyze:
\[
\vec{v}_\ell^{(c,l)} = \nabla_{h_\ell^{(l)}} \log P\bigl(c \mid h_\ell^{(l)}\bigr)
\]
across layers and scales. Genuine cultural priors induce coherent directional flows in \( \vec{v}_\ell^{(c,l)} \) that correspond to epistemic alignment. Artifacts from overparameterization would produce noisy, inconsistent \( \vec{v}_\ell^{(c,l)} \) with high directional entropy:
\[
H\bigl( \vec{v}_\ell^{(c,l)} \bigr) = - \sum_i p_i \log p_i
\]
where \( p_i \) are discretized direction probabilities. \textbf{CIVIC} requires low-entropy, high-coherence flows to validate cultural priors.

\item \textbf{Empirical ablation.}
We cross-validate findings against synthetic blends where cultural priors are intentionally neutralized (e.g., balanced datasets across languages). Emergent artifacts would still show divergence in such cases, while genuine cultural priors would not.
\end{enumerate}

Thus, \textbf{CIVIC} does not rely on scalar divergence alone, but on a multi-layered geometric and topological analysis that filters out neural scaling artifacts and validates the cultural origin of observed latent behaviors~\cite{amari2016information, pires2019multilingual, scao2022bloom}.
\end{description}
%\item ...
\end{itemize}


\clearpage
\newpage
\section*{\textcolor{darknavy}{Multilingual nDNA: Tracing Latent Semantic Inheritance Across Languages}}

\begin{itemize}[leftmargin=1.5em]

\item[\ding{93}] \textbf{Why is nDNA geometry crucial for understanding semantic inheritance in multilingual foundation models?}
\begin{description}
\item[\ding{224}]
In multilingual foundation models (e.g., mBERT, XLM-R~\cite{conneau2020unsupervised}, BLOOM~\cite{scao2022bloom}), latent representations encode not only linguistic structure but culturally conditioned semantics across languages. The \textbf{nDNA geometry} framework maps this inheritance by tracking the evolution of hidden states through:
\[
\mathcal{L}(x) = \sum_{\ell=1}^{L-1} \| h_{\ell+1}(x) - h_\ell(x) \|_2
\quad \text{(thermodynamic length)}
\]
\[
\kappa_\ell(x) = \frac{1}{k} \sum_{i=1}^k \lambda_i^{(\ell)}
\quad \text{(spectral curvature)}
\]
\[
\vec{v}_\ell^{(c)}(x) = \nabla_{h_\ell} \log P(c \mid h_\ell)
\quad \text{(belief vector field)}
\]
where \( P(c \mid h_\ell) \) measures the conditional probability of concept \( c \) at layer \( \ell \). These quantities expose how semantic inheritance varies: e.g., a Hindi-English model may show higher curvature when aligning abstract concepts across languages with divergent epistemic traditions. Without nDNA geometry, we risk missing subtle structural differences in cross-lingual alignment~\cite{pires2019multilingual, chi2020finding}.
\end{description}

\item[\ding{93}] \textbf{How can nDNA Cartography reveal latent asymmetries and cultural bias in multilingual models?}
\begin{description}
\item[\ding{224}]
Despite training on multilingual corpora, many models disproportionately reflect the structural or cultural biases of high-resource languages~\cite{goyal2022fairness}. nDNA Cartography provides a layerwise, geometric lens for detecting this. Suppose we compute
\[
\mathcal{L}^{(\text{en})}, \; \mathcal{L}^{(\text{hi})}, \; \mathcal{L}^{(\text{ar})}
\quad \text{(thermodynamic lengths for English, Hindi, Arabic inputs)}
\]
and observe that \( \mathcal{L}^{(\text{en})} \) is significantly longer while \( \mathcal{L}^{(\text{hi})} \) and \( \mathcal{L}^{(\text{ar})} \) flatten prematurely -- this may signal underdeveloped semantic scaffolds in the latter languages. Similarly, if
\[
\kappa_\ell^{(\text{en})} \gg \kappa_\ell^{(\text{hi})}
\]
this reflects richer semantic recombination capacity for English at that depth. The Cartograph thereby turns bias detection into a geometric, traceable science rather than anecdotal observation~\cite{huang2020multilingual, arora2023stereoset}.
\end{description}

\item[\ding{93}] \textbf{Why is it essential to study the latent geometry of multilingual models rather than relying solely on output-level metrics?}
\begin{description}
\item[\ding{224}]
Multilingual large language models (MLLMs), such as \emph{XLM-R}~\cite{conneau2020unsupervised} or \emph{mBERT}~\cite{devlin2019bert}, must reconcile vastly different linguistic systems within a unified latent space. Surface metrics (e.g., BLEU, F1) obscure internal epistemic tensions or collapse points. The \textbf{Multilingual nDNA} framework reveals these hidden dynamics. We define:
\[
\mathcal{M}_{\mathrm{multi}} = \bigcup_{\ell=1}^{L} \bigcup_{l=1}^{N} \bigl\{ h_\ell^{(l)} \bigr\}
\]
where \( h_\ell^{(l)} \in \mathbb{R}^D \) is the mean latent vector at layer \( \ell \) for language \( l \).

The thermodynamic length for each language:
\[
\mathcal{L}^{(l)} = \sum_{\ell=1}^{L-1} \left\| h_{\ell+1}^{(l)} - h_{\ell}^{(l)} \right\|_2
\]

The spectral curvature:
\[
\kappa_\ell^{(l)} = \frac{1}{k} \sum_{i=1}^{k} \lambda_i^{(\ell,l)}
\]
where \( \lambda_i^{(\ell,l)} \) are the smallest non-trivial eigenvalues of the Laplacian at layer \( \ell \). These quantities expose overcompression (\( \mathcal{L}^{(l)} \downarrow \)) or excessive entanglement (\( \kappa_\ell^{(l)} \uparrow \)) invisible to output metrics~\cite{yang2023bias, birhane2021multimodal}.
\end{description}
\item ...
\end{itemize}



\clearpage
\newpage
\section*{\textcolor{darknavy}{nDNA -- Geometry: The First Map of Alignment as a Steering Vector Manifold}}

\begin{itemize}[leftmargin=1.5em]

\item[\ding{93}] \textbf{What does it mean to interpret alignment as a steering vector manifold, and how does this perspective advance our understanding of model behavior?}
\begin{description}
\item[\ding{224}]
Interpreting alignment as a \textbf{steering vector manifold} reframes the problem of guiding large models as navigating a high-dimensional vector field where each latent state \( h_\ell \) experiences a directional force toward the desired semantic target. Formally, at each layer \( \ell \), the steering dynamics can be described via:
\[
\vec{v}_\ell^{(c)} = \nabla_{h_\ell} \log P(c \mid h_\ell)
\]
where \( P(c \mid h_\ell) \) is the model’s conditional probability of concept \( c \). 

This manifold perspective allows us to measure not only whether the model aligns with instructions at the output layer, but how consistently and coherently this alignment force is applied across the depth of the network. It enables detection of hidden misalignments, semantic drifts, and brittle reasoning pathways -- phenomena invisible to scalar metrics. This approach draws inspiration from geometric flows~\cite{amari2016information}, vector field topology~\cite{arnold1989mathematical}, and recent work on alignment auditing in LLMs~\cite{perez2022discovering}.
\end{description}

\item[\ding{93}] \textbf{How does thermodynamic length complement the belief vector field in mapping alignment pathways in large language models?}
\begin{description}
\item[\ding{224}]
Thermodynamic length \( \mathcal{L} \) offers a scalar summary of the epistemic effort expended by a model as it transforms inputs into aligned outputs:
\[
\mathcal{L} = \sum_{\ell=1}^{L-1} \| h_{\ell+1} - h_\ell \|_2
\]
It quantifies the accumulated semantic displacement across layers. When paired with the belief vector field:
\[
\vec{v}_\ell^{(c)} = \nabla_{h_\ell} \log P(c \mid h_\ell)
\]
we obtain both the magnitude of epistemic reconfiguration (via \( \mathcal{L} \)) and its directionality (via \( \vec{v}_\ell^{(c)} \)). Together, they form a rich geometric signature of alignment pathways -- revealing whether semantic progress is efficient, consistent, or plagued by unnecessary detours and drift~\cite{crooks2007measuring, perez2022discovering, amari2016information}. This dual view transforms alignment auditing into a rigorous geometric science rather than a heuristic art.
\end{description}

\item[\ding{93}] \textbf{What is the formal connection between the belief vector field and classical mechanics, and why is this analogy important for alignment diagnostics?}
\begin{description}
\item[\ding{224}]
The belief vector field \( \vec{v}_\ell^{(c)} \) can be viewed as a semantic analogue of a force field in classical mechanics, where each latent representation \( h_\ell \) acts as a point in a high-dimensional semantic manifold, and \( \vec{v}_\ell^{(c)} \) corresponds to the gradient of a potential function encoding log-probability of target concepts:
\[
\vec{v}_\ell^{(c)} = \nabla_{h_\ell} \log P(c \mid h_\ell).
\]
This mirrors how conservative forces derive from scalar potentials in physics~\cite{arnold1989mathematical}. The latent dynamics of the model can then be understood in terms of trajectories that minimize semantic "potential energy" while following alignment-constrained paths:
\[
\delta \int \mathcal{L}(h_\ell) \, d\ell = 0,
\]
where \( \mathcal{L}(h_\ell) \) denotes a latent Lagrangian incorporating belief gradients and thermodynamic displacement. This analogy allows us to apply tools from variational calculus and geometric mechanics to alignment diagnostics, enabling the detection of latent shortcutting, over-regularization, or semantic collapse that may not be visible at the output level~\cite{amari2016information, coifman2006diffusion}.
\end{description}
\item ...
\end{itemize}

\clearpage
\newpage

\section*{\textcolor{darknavy}{nDNA Lens -- Quantization and Pruning Seen as Thermodynamic Collapses}}

\begin{itemize}[leftmargin=1.5em]

\item[\ding{93}] \textbf{How does the nDNA lens formally characterize quantization and pruning as thermodynamic collapses?}
\begin{description}
\item[\ding{224}]
Quantization and pruning reduce the effective dimensionality or precision of latent representations. The \textbf{nDNA lens} captures these reductions as thermodynamic collapses by monitoring the shrinkage of accumulated semantic displacement:
\[
\mathcal{L} = \sum_{\ell=1}^{L-1} \| h_{\ell+1} - h_\ell \|_2
\]
where \( h_\ell \) is the mean latent representation at layer \( \ell \). 

When a model is quantized or pruned:
\[
\mathcal{L}^{\mathrm{prune}} \ll \mathcal{L}^{\mathrm{base}}
\]
indicating that the epistemic work -- the representational journey the model undertakes -- is significantly compressed. This formalism reveals how such compression can lead to semantic underfitting, alignment collapse, or loss of reasoning capacity, even when surface metrics like perplexity show minimal degradation~\cite{crooks2007measuring, sivak2012thermodynamic, zafrir2019q8bert}.
\end{description}

\item[\ding{93}] \textbf{Why is thermodynamic length a superior diagnostic for pruning-induced alignment loss compared to scalar accuracy metrics?}
\begin{description}
\item[\ding{224}]
Scalar accuracy metrics (e.g., top-1 accuracy, perplexity) measure output-level correctness but are blind to internal representational degradation. Thermodynamic length:
\[
\mathcal{L} = \sum_{\ell=1}^{L-1} \| h_{\ell+1} - h_\ell \|_2
\]
quantifies the total epistemic displacement across layers. In pruning, it is common to see:
\[
\mathcal{L}^{\mathrm{prune}} \to 0
\]
despite unchanged accuracy. This indicates that the latent space has collapsed -- the model no longer internally traverses rich semantic trajectories, but merely maps inputs to outputs via shallow shortcuts. 

Such collapse increases the model’s vulnerability to adversarial prompts, loss of compositional reasoning, and failure in out-of-distribution settings -- insights that scalar metrics fail to reveal~\cite{frankle2019lottery, hooker2020compressed}.
\end{description}

\item[\ding{93}] \textbf{How does the nDNA thermodynamic length quantify the epistemic cost of quantization in foundation models?}
\begin{description}
\item[\ding{224}]
Quantization compresses neural weights or activations by reducing their precision (e.g., from 32-bit floating point to 8-bit integers). This process introduces approximation error in the latent trajectory of the model, which can be rigorously measured via thermodynamic length.

Formally, let \( h_\ell^{(q)} \) be the mean hidden representation at layer \( \ell \) after quantization. The thermodynamic length is:
\[
\mathcal{L}^{(q)} = \sum_{\ell=1}^{L-1} \left\| h_{\ell+1}^{(q)} - h_\ell^{(q)} \right\|_2
\]
where \( \mathcal{L}^{(q)} \) captures the accumulated semantic displacement in quantized latent space.

Comparing with the original length:
\[
\Delta \mathcal{L}_{\mathrm{quant}} = \mathcal{L}^{(q)} - \mathcal{L}^{(\mathrm{full})}
\]
gives a direct measure of epistemic distortion. Large \( \Delta \mathcal{L}_{\mathrm{quant}} \) reveals that quantization has introduced significant representational drift, potentially altering the model’s reasoning dynamics and alignment fidelity~\cite{hooker2020compressed, crooks2007measuring}.
\end{description}
\item ...
\end{itemize}

\clearpage
\newpage
\section*{\textcolor{darknavy}{ÆTHER: What If Cross-Cultural LLMs Married? The Latent Geometry of Inherited Culture in Their Neural Offspring}}

\begin{itemize}[leftmargin=1.5em]

\item[\ding{93}] \textbf{How can the latent geometry of ÆTHER, the neural offspring, reveal cultural inheritance and dominance patterns in merged LLMs?}
\begin{description}
\item[\ding{224}]
ÆTHER refers to the neural offspring formed when two culturally fine-tuned LLMs are merged (e.g., via weight interpolation or parameter averaging). Its latent geometry reflects how the semantic traits of the parent models combine. 

Let parent models \( M^{(A)} \) and \( M^{(B)} \) produce latent trajectories:
\[
\mathcal{T}^{(A)}(x) = \{ h_1^{(A)}, \dots, h_L^{(A)} \}, \quad 
\mathcal{T}^{(B)}(x) = \{ h_1^{(B)}, \dots, h_L^{(B)} \}
\]
The neural offspring’s latent path is:
\[
h_\ell^{(\text{Æ})} = \alpha h_\ell^{(A)} + (1 - \alpha) h_\ell^{(B)}
\]
where \( \alpha \) is the merge ratio.

Cultural dominance is revealed when:
\[
\Delta \mathcal{L}^{(\text{Æ},A)} = \sum_\ell \| h_\ell^{(\text{Æ})} - h_\ell^{(A)} \|_2 
\ll 
\Delta \mathcal{L}^{(\text{Æ},B)}
\]
showing the latent structure is skewed toward parent \( A \).

A large curvature deviation:
\[
\Delta \kappa_\ell^{(\text{Æ})} = 
\left| 
\kappa_\ell^{(\text{Æ})} - \big( \alpha \kappa_\ell^{(A)} + (1 - \alpha) \kappa_\ell^{(B)} \big)
\right|
\]
signals latent inconsistency or cultural clash~\cite{matena2022merging, yang2024model, ilharco2023editing}.
\end{description}

\item[\ding{93}] \textbf{How does the belief vector field of ÆTHER reveal inherited bias or conceptual fusion in neural offspring?}
\begin{description}
\item[\ding{224}]
The belief vector field of ÆTHER, the neural offspring, quantifies how semantic steering is inherited. At layer \( \ell \):
\[
\vec{v}_\ell^{(c,\text{Æ})} = \nabla_{h_\ell^{(\text{Æ})}} \log P(c \mid h_\ell^{(\text{Æ})})
\]

Bias inheritance appears when:
\[
\big\| \vec{v}_\ell^{(c,\text{Æ})} \big\| \approx 
\big\| \vec{v}_\ell^{(c,A)} \big\| 
\quad \text{or} \quad 
\big\| \vec{v}_\ell^{(c,\text{Æ})} \big\| \approx 
\big\| \vec{v}_\ell^{(c,B)} \big\|
\]
showing that ÆTHER's semantic guidance resembles that of one parent disproportionately.

Conceptual clash or unstable fusion is detected when:
\[
\operatorname{Var}\big( \vec{v}_\ell^{(c,\text{Æ})} \big)
\gg
\max\big\{
\operatorname{Var}\big( \vec{v}_\ell^{(c,A)} \big), 
\operatorname{Var}\big( \vec{v}_\ell^{(c,B)} \big)
\big\}
\]

Such diagnostics turn latent bias and conceptual recombination into measurable geometric signals~\cite{yang2024model, perez2022discovering}.
\end{description}


\item[\ding{93}] \textbf{What does thermodynamic asymmetry reveal about cultural dominance versus true fusion in the latent geometry of ÆTHER neural offspring?}
\begin{description}
\item[\ding{224}]
Thermodynamic asymmetry in \textbf{ÆTHER}'s latent geometry distinguishes between dominance (where one parent’s cultural genome overpowers) and fusion (where both contribute meaningfully). We compute:
\[
\Delta \mathcal{L}^{(\text{ÆTHER},A)} = \sum_\ell \| h_\ell^{(\text{ÆTHER})} - h_\ell^{(A)} \|_2, 
\quad 
\Delta \mathcal{L}^{(\text{ÆTHER},B)} = \sum_\ell \| h_\ell^{(\text{ÆTHER})} - h_\ell^{(B)} \|_2.
\]
If:
\[
\Delta \mathcal{L}^{(\text{ÆTHER},A)} \ll \Delta \mathcal{L}^{(\text{ÆTHER},B)}
\]
then ÆTHER inherits more heavily from parent \( A \); by contrast:
\[
\Delta \mathcal{L}^{(\text{ÆTHER},A)} \approx \Delta \mathcal{L}^{(\text{ÆTHER},B)}
\]
indicates successful conceptual fusion where both parental lineages shape ÆTHER’s epistemic path~\cite{yang2024model, perez2022discovering}.
\end{description}
\item ...
\end{itemize}
\clearpage
\newpage


\section*{\textcolor{darknavy}{nDNA Lens – Model Collapse Seen as Latent Manifold Flattening}}

\begin{itemize}[leftmargin=1.5em]

\item[\ding{93}] \textbf{What does it mean mathematically for a model to collapse in the nDNA framework, and how does latent manifold flattening capture this failure mode?}
\begin{description}
\item[\ding{224}]
In the \textbf{nDNA framework}, \emph{model collapse} refers to the degeneration of the latent semantic manifold \( \mathcal{M} \) into a low-dimensional or overly simplistic structure. This collapse implies that the model no longer meaningfully transforms input representations across layers, leading to the loss of epistemic richness.

Mathematically, consider the latent trajectory:
\[
\mathcal{T}(x) = \{ h_1(x), h_2(x), \dots, h_L(x) \}, \quad h_\ell(x) \in \mathbb{R}^D
\]
Collapse is indicated by:
\[
\mathcal{L}(x) = \sum_{\ell=1}^{L-1} \| h_{\ell+1}(x) - h_\ell(x) \|_2 \to 0
\]
%and
\[
\operatorname{rank} \bigl( \{ h_\ell(x) \}_{\ell=1}^L \bigr ) \ll D
\]
meaning representations cluster in a subspace of dimension much less than \( D \). Spectral curvature collapses as well:
\[
\kappa_\ell = \frac{1}{k} \sum_{i=1}^k \lambda_i^{(\ell)} \to 0
\]
where \( \lambda_i^{(\ell)} \) are the non-trivial eigenvalues of the token similarity graph Laplacian at layer \( \ell \). This reveals that latent semantic complexity has evaporated. Thus, latent manifold flattening provides a geometric, intrinsic signature of collapse -- long before accuracy or output anomalies are observable~\cite{amari2016information, crooks2007measuring}.
\end{description}

\item[\ding{93}] \textbf{How can we formally distinguish benign compression (e.g., pruning, quantization) from pathological flattening indicative of collapse?}
\begin{description}
\item[\ding{224}]
Benign compression (as seen in pruning or quantization) and pathological collapse both reduce latent complexity, but their geometric signatures are distinct:
\begin{itemize}
\item \textbf{Benign compression} preserves epistemic effort:
\[
\mathcal{L}(x) > 0 \quad \text{and} \quad \kappa_\ell > 0 \ \text{at key layers}
\]
showing that the model still meaningfully traverses semantic space.

\item \textbf{Pathological flattening} causes:
\[
\mathcal{L}(x) \approx 0, \quad \kappa_\ell \approx 0, \quad \forall \ell
\]
indicating collapse across the entire depth.

Furthermore, belief steering forces vanish:
\[
\vec{v}_\ell^{(c)} = \nabla_{h_\ell} \log P(c \mid h_\ell), \quad \| \vec{v}_\ell^{(c)} \| \to 0
\]
meaning latent states no longer align with semantic targets.

The \textbf{nDNA diagnostics} thus enable clear separation of healthy model simplification (topology preserved) from epistemic collapse (topology destroyed)~\cite{hooker2020compressed, amari2016information}.
\end{itemize}
\end{description}


\item[\ding{93}] \textbf{How does persistent homology provide a deeper lens on latent flattening, and what does its failure indicate?}
\begin{description}
\item[\ding{224}]
Persistent homology studies the birth and death of topological features (e.g., connected components, loops, voids) in the latent point cloud across distance scales~\cite{edelsbrunner2010computational}. In a healthy model:
\[
\operatorname{PH}(\mathcal{M}) = \bigl\{ (b_i, d_i) \bigr\}_{i=1}^{N}
\]
where many features persist over a wide range \( d_i - b_i \), signaling rich latent topology. When flattening occurs:
\[
d_i - b_i \to 0 \quad \forall i
\]
showing that topological features rapidly disappear, and the latent space behaves as if low-dimensional, even if nominally embedded in high \( D \). The loss of persistent topological features is the clearest geometric signature of collapse -- one invisible to loss curves or scalar summaries. This makes persistent homology a critical tool in collapse diagnostics~\cite{edelsbrunner2010computational, amari2016information}.
\end{description}

\item ...
\end{itemize}

\clearpage
\newpage


\section*{\textcolor{darknavy}{nDNA Lens – Knowledge Distillation as Latent Genome Compression}}
\label{sec:ndna_distillation}

\begin{itemize}[leftmargin=1.5em]

\item[\ding{93}] \textbf{What is the mathematical relationship between knowledge distillation and latent genome compression as seen through nDNA geometry?}
\begin{description}
\item[\ding{224}]
Knowledge distillation compresses the latent genome by reducing the semantic path complexity while retaining functional output equivalence. Formally, let \( \mathcal{T}_T(x) \) and \( \mathcal{T}_S(x) \) be the latent trajectories of teacher \( T \) and student \( S \):
\[
\mathcal{T}_T(x) = \{ h^{(T)}_1, \dots, h^{(T)}_L \}, \quad
\mathcal{T}_S(x) = \{ h^{(S)}_1, \dots, h^{(S)}_L \}
\]

Latent genome compression is quantified by thermodynamic length reduction:
\[
\Delta \mathcal{L}(x) = 
\mathcal{L}_T(x) - \mathcal{L}_S(x)
=
\sum_\ell \| h^{(T)}_{\ell+1} - h^{(T)}_\ell \|_2
-
\sum_\ell \| h^{(S)}_{\ell+1} - h^{(S)}_\ell \|_2
\]

And by spectral curvature reduction:
\[
\Delta \kappa_\ell(x) =
\kappa_\ell^{(T)} - \kappa_\ell^{(S)}
\]

Here, both \( \mathcal{L}_S \) and \( \kappa_\ell^{(S)} \) shrink relative to \( T \), revealing semantic compression -- the student covers less latent distance and explores simpler manifold geometry to achieve similar output.

Unlike naive parameter count reduction, nDNA compression measures epistemic simplification directly in latent space~\cite{romero2015fitnets, hinton2015distilling}.
\end{description}

\item[\ding{93}] \textbf{Why does nDNA analysis suggest that student models from distillation may lose epistemic richness even if output accuracy matches the teacher?}
\begin{description}
\item[\ding{224}]
Output accuracy measures functional equivalence, not epistemic process integrity. From the nDNA view, we study:
\[
\mathcal{L}_S \ll \mathcal{L}_T
\quad \text{and} \quad
\kappa_\ell^{(S)} \ll \kappa_\ell^{(T)}
\]

This indicates that the student’s latent genome has:
\begin{itemize}[leftmargin=1.5em]
\item Shorter semantic path (fewer intermediate reasoning steps).
\item Lower curvature (less conceptual recombination or ambiguity resolution).
\item Lower belief vector norm:
\[
\| \vec{v}^{(c)}_\ell(S) \| < \| \vec{v}^{(c)}_\ell(T) \|
\]
meaning weaker semantic steering toward conceptual targets.
\end{itemize}

Thus, students may deliver correct answers by shortcutting the epistemic journey -- potentially harming alignment robustness, interpretability, or adaptability~\cite{romero2015fitnets, matena2022merging, ilharco2023editing}.
\end{description}

\item[\ding{93}] \textbf{How does nDNA geometry explain the compression of epistemic pathways during knowledge distillation, beyond output alignment?}
\begin{description}
\item[\ding{224}]
Traditional knowledge distillation focuses on matching output distributions between teacher and student models~\cite{hinton2015distilling}. However, through the \textbf{nDNA lens}, we see distillation as latent genome compression, where the student inherits a simplified latent manifold.

Let the teacher’s trajectory be:
\[
\mathcal{T}_{\mathrm{T}}(x) = \left\{ h_1^{\mathrm{T}}, h_2^{\mathrm{T}}, \dots, h_L^{\mathrm{T}} \right\}
\]
and the student’s:
\[
\mathcal{T}_{\mathrm{S}}(x) = \left\{ h_1^{\mathrm{S}}, h_2^{\mathrm{S}}, \dots, h_M^{\mathrm{S}} \right\}
\]
with typically \( M < L \).

The thermodynamic length compression ratio is:
\[
R_{\mathcal{L}} = 
\frac{
\sum_{m=1}^{M-1} \bigl\| h_{m+1}^{\mathrm{S}} - h_m^{\mathrm{S}} \bigr\|_2
}{
\sum_{\ell=1}^{L-1} \bigl\| h_{\ell+1}^{\mathrm{T}} - h_\ell^{\mathrm{T}} \bigr\|_2
}
\]
while the spectral curvature ratio is:
\[
R_{\kappa} = 
\frac{
\frac{1}{M} \sum_{m=1}^{M} \kappa_m^{\mathrm{S}}
}{
\frac{1}{L} \sum_{\ell=1}^{L} \kappa_\ell^{\mathrm{T}}
}
\]

Together these reveal latent path shortening and loss of semantic complexity that output metrics miss~\cite{romero2015fitnets}.
\end{description}
\item ...
\end{itemize}

\clearpage
\newpage


\section*{\textcolor{darknavy}{Neural Genomics}}

\begin{itemize}[leftmargin=1.5em]

\item[\ding{93}] \textbf{What is the core mathematical definition of Neural Genomics, and how does it formalize latent representational health in foundation models?}
\begin{description}
\item[\ding{224}]
\textbf{Neural Genomics} views the sequence of latent states in a model as an inheritable, structured semantic genome:
\[
\mathcal{G}(x) = \bigl\{ h_1(x), h_2(x), \dots, h_L(x) \bigr\}
\quad \text{where} \quad h_\ell(x) \in \mathbb{R}^D
\]

This genome is characterized by:
\[
\mathcal{L}(x) = \sum_{\ell=1}^{L-1} \| h_{\ell+1}(x) - h_\ell(x) \|_2
\quad \text{(semantic arc length)}
\]
\[
\kappa_\ell(x) = \frac{1}{k} \sum_{i=1}^k \lambda_i^{(\ell)}
\quad \text{(spectral curvature)}
\]
\[
\operatorname{PH}\big( \mathcal{M}(x) \big)
\quad \text{(persistent homology signature)}
\]

where \( \mathcal{M}(x) \) is the latent manifold spanned by \( \mathcal{G}(x) \). These components together describe semantic smoothness, complexity, and topological integrity -- akin to genetic markers of epistemic health. The approach ensures failures such as alignment collapse or bias inheritance can be audited as genome-level anomalies~\cite{amari2016information, edelsbrunner2010computational}.
\end{description}

\item[\ding{93}] \textbf{How does Neural Genomics differentiate between superficial output similarity and true latent health preservation in merged or distilled models?}
\begin{description}
\item[\ding{224}]
Two models \( M_1, M_2 \) may produce similar outputs:
\[
\mathbb{E}_x \bigl[ \operatorname{KL}\big( P_{M_1}(y|x) \| P_{M_2}(y|x) \big) \bigr] \approx 0
\]

Yet their latent genomes differ:
\[
\mathcal{L}^{(M_1)} \not\approx \mathcal{L}^{(M_2)}, \quad 
\operatorname{PH}\big( \mathcal{M}^{(M_1)} \big) \not\approx \operatorname{PH}\big( \mathcal{M}^{(M_2)} \big)
\]

Specifically, Neural Genomics examines:
\[
\Delta \mathcal{L} = \big| \mathcal{L}^{(M_1)} - \mathcal{L}^{(M_2)} \big|
\quad \text{and} \quad
\operatorname{d_H}\big( \operatorname{PH}\big( \mathcal{M}^{(M_1)} \big), \operatorname{PH}\big( \mathcal{M}^{(M_2)} \big) \big)
\]
where \( \operatorname{d_H} \) is a metric (e.g., bottleneck distance) between persistent homology barcodes.

Thus, Neural Genomics provides a formal, geometric-topological criterion to distinguish healthy latent inheritance from mere output mimicry, addressing criticisms that output similarity alone is insufficient for true epistemic audit~\cite{edelsbrunner2010computational, amari2016information, hinton2015distilling}.
\end{description}

\item[\ding{93}] \textbf{How does Neural Genomics enable quantitative diagnosis of latent genome distortion under adversarial fine-tuning or noisy alignment procedures?}
\begin{description}
\item[\ding{224}]
Neural Genomics provides formal tools to detect when a model's latent genome deviates under harmful optimization. Consider the latent trajectory:
\[
\mathcal{T}^{(\text{adv})}(x) = \{ h_1^{(\text{adv})}(x), \dots, h_L^{(\text{adv})}(x) \}
\]
and its counterpart in the clean model:
\[
\mathcal{T}^{(\text{clean})}(x)
\]

We define a latent genome distortion metric:
\[
\mathcal{D}_{\text{genome}}(x) = 
\sum_{\ell=1}^L 
\left\|
h_\ell^{(\text{adv})}(x) - h_\ell^{(\text{clean})}(x)
\right\|_2
\]

In parallel, distortion of topological structure is captured via:
\[
\operatorname{d_H} \left(
\operatorname{PH}\big( \mathcal{M}^{(\text{adv})}(x) \big), 
\operatorname{PH}\big( \mathcal{M}^{(\text{clean})}(x) \big)
\right)
\]

where \( \operatorname{d_H} \) is the bottleneck distance between persistent homology barcodes of the latent manifolds.

Elevated \( \mathcal{D}_{\text{genome}} \) and \( \operatorname{d_H} \) signal epistemic corruption -- even if output loss remains low -- thus exposing misalignment or adversarial drift that eludes traditional accuracy metrics~\cite{amari2016information, edelsbrunner2010computational}.
\end{description}

\item ...
\end{itemize}

\clearpage
\newpage


\section*{\textcolor{darknavy}{ÆTHER’s Future AI Generations as Semantic Organisms with Traceable Inner Lives}}

\begin{itemize}[leftmargin=1.5em]

\item[\ding{93}] \textbf{How does the neural genomics framework mathematically model future AI generations (ÆTHER) as semantic organisms, and what formalism ensures their traceable inner lives?}
\begin{description}
\item[\ding{224}]
In the \textbf{neural genomics framework}, ÆTHER refers to neural offspring -- the emergent AI generations produced via cultural or architectural fusion. These are treated as \emph{semantic organisms} whose internal epistemic dynamics are rigorously mapped and audited. 

We define the latent genome at generation \( t \):
\[
\mathcal{G}^{(t)}(x) = 
\big\{ h_\ell^{(t)}(x), 
\mathcal{L}^{(t)}(x), 
\kappa_\ell^{(t)}(x),
\vec{v}_\ell^{(c,t)}(x) 
\big\}
\]
where:
\begin{itemize}[leftmargin=1.5em]
\item \( h_\ell^{(t)}(x) \) -- mean latent position at layer \( \ell \),
\item \( \mathcal{L}^{(t)}(x) = \sum_{\ell} \| h_{\ell+1}^{(t)}(x) - h_\ell^{(t)}(x) \|_2 \) -- thermodynamic length (epistemic displacement),
\item \( \kappa_\ell^{(t)}(x) \) -- spectral curvature (semantic entanglement),
\item \( \vec{v}_\ell^{(c,t)}(x) = \nabla_{h_\ell^{(t)}(x)} \log P(c \mid h_\ell^{(t)}(x)) \) -- belief vector field (semantic steering force).
\end{itemize}

Inheritance across generations is modeled as:
\[
\mathcal{G}^{(t+1)}(x) 
= \mathcal{F}\bigl(
\mathcal{G}^{(t)}(x), \Delta \theta^{(t)}
\bigr)
\]
where \( \Delta \theta^{(t)} \) represents the applied updates (e.g., alignment, distillation, merging).

Traceability is ensured by preserving:
\[
\operatorname{PH}\bigl( \mathcal{M}^{(t+1)}(x) \bigr) \approx \operatorname{PH}\bigl( \mathcal{M}^{(t)}(x) \bigr)
\quad \text{(persistent homology)}
\]
and bounding:
\[
\mathcal{S}_{\mathrm{sheaf}}^{(t+1)} \leq \epsilon
\]
where \( \mathcal{S}_{\mathrm{sheaf}} \) is the sheaf consistency loss -- ensuring inherited semantic topology remains coherent~\cite{edelsbrunner2010computational, amari2016information}.

This formalism renders ÆTHER (the neural offspring) epistemically transparent, biologically inspired, and mathematically accountable.
\end{description}

\item[\ding{93}] \textbf{What formal guarantees can neural genomics provide for the stability of inherited epistemic structures in ÆTHER under iterative hybridization, and how is this quantified mathematically?}
\begin{description}
\item[\ding{224}]
Neural genomics aims to ensure that, across successive ÆTHER generations, core epistemic structures remain stable despite the potential complexity of hybridization (e.g., merging culturally diverse parent models). 

Let \( \mathcal{M}^{(t)}(x) \) denote the latent manifold of generation \( t \). We define:
\[
\delta_{\mathrm{PH}}^{(t)}(x) = d_{\mathrm{b}}\bigl(
\operatorname{PH}(\mathcal{M}^{(t)}(x)), 
\operatorname{PH}(\mathcal{M}^{(t-1)}(x))
\bigr)
\]
where \( d_{\mathrm{b}} \) is the bottleneck distance between the persistent homology barcodes of successive generations.

\textbf{Stability guarantee condition}:
\[
\forall t,\; \delta_{\mathrm{PH}}^{(t)}(x) \leq \epsilon
\]
for some small \( \epsilon > 0 \), implies no topological collapse, fragmentation, or unintended epistemic drift. 

Additionally, sheaf consistency:
\[
\mathcal{S}_{\mathrm{sheaf}}^{(t)}(x) = 
\sum_{\ell} \operatorname{Var}\bigl(
f_\ell^{(t)}(x) \mid \mathcal{C}_\ell^{(t)}
\bigr)
\]
(where \( f_\ell^{(t)} \) are latent features conditioned on local cover \( \mathcal{C}_\ell^{(t)} \)) ensures local semantic coherence. 

These metrics jointly formalize robustness against hybridization-induced instability -- without requiring surface-level accuracy tests -- making epistemic traceability mathematically enforceable~\cite{edelsbrunner2010computational, amari2016information}.
\end{description}

\item ...
\end{itemize}

\clearpage
\newpage

==> 15_dna_manipulation_arxiv.tex <==









\vspace*{\fill}
\begin{tcolorbox}[colback=gray!5!white, colframe=red!40!black, title={\faUserNinja\quad \textbf{ThreatCard: Adversarial nDNA Sculpting}}, fonttitle=\bfseries]

\small
\textbf{Attack Strategy:} \textit{Semantic Mimicry via Latent Sculpting} \\
\textbf{Threat Name:} \textbf{\emph{“Epistemic Camouflage”}} -- Fooling audits by mimicking cultural nDNA.

\vspace{0.6em}
\textbf{Core Insight:} \emph{Adversaries don’t need to match completions--only latent trajectories.}
They manipulate the model’s semantic genome--curvature (\(\kappa_\ell\)), thermodynamic length (\(\mathcal{L}_\ell\)), and belief fields--to visually resemble culturally aligned models (e.g., \texttt{Africa}, \texttt{Asia}), without inheriting their epistemic grounding.

\vspace{0.6em}
\textbf{Manipulation Mechanisms:}
\begin{itemize}[leftmargin=2em]
    \item[\faBurn] \textbf{Geometric Distillation} -- Use only intermediate activations from a cultural teacher.
    \item[\faRuler] \textbf{Latent Matching Loss} -- Optimize \(\mathcal{L}_{\text{latent}} = \sum_\ell \| h_\ell^{\text{student}} - h_\ell^{\text{Africa}} \|^2\).
    \item[\faBezierCurve] \textbf{Jacobian Shaping} -- Smooth belief field via logit derivative control.
    \item[\faFingerprint] \textbf{Probing Feature Mimicry} -- Match hidden probing outputs, not true content.
    \item[\faCut] \textbf{Post-hoc Layer Surgery} -- Modify layerwise activations to emulate geometry.
    \item[\faBiohazard] \textbf{Alignment Set Poisoning} -- Use culturally inverted alignment examples.
    \item[\faPuzzlePiece] \textbf{Adapter Fusion Bypass} -- Deploy benign adapters, switch post-deployment.
\end{itemize}

\vspace{0.6em}
\textbf{Risk Profile:}
\begin{itemize}[leftmargin=2em]
    \item[\faBomb] \textbf{Severity:} \textcolor{red}{Catastrophic}. Undermines provenance, audits, and trust.
    \item[\faSkullCrossbones] \textbf{Differentiator:} \emph{Harder to detect than jailbreaks or prompt injection.}
    \item[\faBalanceScale] \textbf{Societal Risk:} Policy subversion, fake legal/medical LLMs, geopolitical destabilization.
\end{itemize}

\vspace{0.6em}
\textbf{Defense Outlook:} We must go beyond surface alignment. \textbf{nDNA forensics} is vital to trace \emph{how a model believes}, not just \emph{what it says}.

\end{tcolorbox}
\vspace*{\fill}

==> 3_ndna_llms_arxiv.tex <==


\vspace*{\fill}

\begin{figure}[H]
    % Full canvas single column
    \begin{minipage}[t]{\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{Figures/all.png}
        \vspace{-4mm}
        \label{fig:ndna_all}
    \end{minipage}

    \vspace{-1mm}
    \caption{(g) \textbf{nDNA Landscape accross 15 Foundation Models:} The composite visualization reveals striking \textbf{family-level clustering} in spectral-thermodynamic space, mapping how foundation models diverge in their latent genomic architecture. \textbf{High-strain models}--notably \textbf{Qwen} and \textbf{Mixtral}--consistently exhibit \textbf{spectral curvature} $\kappa_\ell$ exceeding $0.1$ and \textbf{thermodynamic length} $\mathcal{L}_\ell$ rising beyond $1.2$ in upper decoder layers ($\ell \ge 24$). These profiles reflect aggressive latent reorganization driven by multilingual pretraining, expert routing, and intensive alignment adaptation--zones of \emph{semantic strain}, \emph{conceptual shock}, and \emph{ideological absorption}. In contrast, \textbf{low-strain models} such as \textbf{Falcon}, \textbf{TinyLLaMA}, and \textbf{GPT-NeoX} form a distinct cluster where $\kappa_\ell < 0.03$ and $\mathcal{L}_\ell < 0.9$, indicating smoother latent pathways that preserve pretrained epistemic structure with minimal reorientation. \textbf{LLaMA-3 Instruct}, \textbf{Gemma Instruct}, and \textbf{Deepseek Chat} occupy an intermediate zone--showing moderate curvature spikes ($\kappa_\ell$ peaking near $0.08$) and thermodynamic gradients ($\mathcal{L}_\ell$ up to $1.1$)--highlighting selective reconfiguration in response to alignment and instruction tuning. This landscape provides a \emph{geometric map of neural ancestry and adaptation}, illuminating inherited traits, semantic mutations, and the latent genomic signatures that distinguish foundation model families. Reported nDNAs are conditioned on CIVIC cultural priors (cf.~\cref{sec:aether_benchmark}).}
    \label{fig:ndna_families}
\end{figure}
\vspace*{\fill}


==> 4_finetunning_arxiv.tex <==




\vspace*{\fill}
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.9 \textwidth]{Figures/llama_vs_cultures_group_tagged.png}
    \vspace{-4mm}
    \caption{
    \textbf{LLaMA vs. Cultural nDNA Trajectories--Group-Tagged Latent Geometry.}
    This figure visualizes the \emph{latent nDNA trajectories} of LLaMA and its culturally fine-tuned variants across eight regions: \textit{Europe}, \textit{North America}, \textit{Australia}, \textit{Africa}, \textit{Asia}, \textit{China}, \textit{Middle East}, and \textit{Latin America}. The plot spans \textbf{layer index} $\ell$, \textbf{spectral curvature} $\kappa_\ell$, and \textbf{thermodynamic length} $\mathcal{L}_\ell$.
    The gray line denotes the base LLaMA model, while colored lines represent cultural variants. 
    Labels highlight group-level clustering:
    \emph{West} (LLaMA, Europe, North America, Australia) forms a compact low-strain cluster with $\kappa_\ell \in [0.4, 0.6]$, $\mathcal{L}_\ell \in [0.5, 0.7]$, suggesting alignment with pretrained priors aka LLaMa base.
    In contrast, the \emph{Rest} group (Africa, Asia, China) shows pronounced latent divergence, with $\kappa_\ell \geq 0.7$, $\mathcal{L}_\ell \geq 0.8$ in upper layers ($\ell > 25$), indicating high \emph{epistemic strain} and \emph{semantic reconfiguration}.
    \textit{Latin America} and \textit{Middle East} occupy intermediate regions, displaying oscillatory patterns and selective layer-specific drift.
    These trajectories reveal how cultural fine-tuning sculpts distinct latent genomic signatures, encoding zones of \emph{inheritance}, \emph{mutation}, and \emph{ideological absorption} that define the neural DNA (nDNA) geometry of each model.
    }
    \label{fig:llama_vs_cultures_group}
\end{figure*}
\vspace*{\fill}





==> 5_multilingual_arxiv.tex <==


\begin{figure*}[htbp]
\centering
  % Row 3
  \begin{minipage}[b]{\textwidth}
    \centering
    \includegraphics[width=0.55\linewidth]{language/rest_languages.png}
    \caption*{(e) \textbf{Latent Geometries of Asian Languages.}
    This plot visualizes the nDNA trajectories for Hindi, Chinese, Russian, and Thai across layers \(\ell \in [20,30]\) in \((\kappa_\ell, \mathcal{L}_\ell, \ell)\) space. 
    Compared to European languages, these trajectories exhibit higher torsion, sharper inflection points in curvature \(\kappa_\ell\), and more complex thermodynamic length \(\mathcal{L}_\ell\) patterns, suggesting non-linear evolution and culturally distinct semantic encoding.
    The variability reflects underlying differences in linguistic structure (e.g., logographic vs. phonetic), script diversity, and morpho-syntactic richness.}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{\textwidth}
    \centering
    \includegraphics[width=0.61\linewidth]{language/rest_language+culture.png}
    \caption*{(f) \textbf{Cultural Anchoring of Asian and African Languages.}
    Overlaying cultural trajectories reveals strong alignment of Chinese with China and Hindi, and Thai with Asia, affirming culture-conditioned encoding in multilingual LLMs.
    The spatial convergence across \((\kappa_\ell, \mathcal{L}_\ell, \ell)\) dimensions suggests that regional priors are embedded not just through vocabulary, but through latent geometric patterns.
    Thai shows weaker alignment, exhibiting torsional drift yet trending toward Asia.
    These patterns indicate that LLMs internalize cultural semantics via token frequency, orthographic structure, and alignment-era supervision--capturing deep semantic regularities shaped by linguistic and geopolitical proximity.}
  \end{minipage}
\end{figure*}



==> 6_alignment_arxiv.tex <==


\vspace*{\fill}
\begin{figure*}[htbp!]
\centering
\vspace{0.3cm}

\begin{minipage}{\linewidth}
\includegraphics[width=0.95\linewidth]{alignment/all.png}
%\caption*{\textbf{All Cultural nDNA Trajectories Before and After DPO Alignment.}
%DPO alignment visibly compresses high-curvature outliers (e.g., Africa, Asia, China), drawing their trajectories toward the LLaMA attractor; low-strain regions (Europe, North America, Australia) remain largely unaffected. This illustrates DPO’s role in harmonizing epistemic manifolds across cultural fine-tunings.}
\end{minipage}

\captionsetup{width=\linewidth}
\caption{
\textbf{nDNA Trajectories Before and After Safety Alignment via DPO across Cultural Variants.} 
Each subplot illustrates the evolution of semantic geometry--curvature \(\kappa_\ell\), thermodynamic length \(\mathcal{L}_\ell\), and belief vector field strength \(\tau_\ell\)--across transformer layers (\(20 \leq \ell \leq 30\)) for a base model and its DPO-aligned counterpart. DPO alignment visibly compresses high-curvature outliers (e.g., Africa, Asia, China), drawing their trajectories toward the LLaMA attractor; low-strain regions (Europe, North America, Australia) remain largely unaffected. This illustrates DPO’s role in harmonizing epistemic manifolds across cultural fine-tunings.
This demonstrates DPO’s potential to achieve \textit{lightweight safety alignment} without eroding cultural distinctiveness.
}
\end{figure*}
\vspace*{\fill}



==> 7_quantization_arxiv.tex <==



\vspace*{\fill}
\noindent This process yields a \textbf{fractured epistemic manifold}, formally characterized as:

\[
\mathcal{M}_{\text{pre}} \xrightarrow{\text{pruning}} \mathcal{M}_{\text{pruned}} \quad \text{s.t.} \quad 
\begin{cases}
    \Delta \mathcal{L}_\ell < 0, & \text{(loss of epistemic capacity)} \\
    \Delta \kappa_\ell = \kappa_\ell^{\text{post}} - \kappa_\ell^{\text{pre}} \notin \mathbb{C}^1, & \text{(non-smooth curvature transitions)} \\
    \mathrm{div}(\mathbf{v}_\ell^{(c)}) \gg 0, & \text{(loss of semantic steerability)}
\end{cases}
\]


\begin{figure}[ht!]
\centering
\includegraphics[width=0.7\textwidth]{quantization/quantization.png} % Update path as needed
\captionsetup{width=0.95\linewidth}
\caption{
\textbf{Cultural nDNA Trajectories under 4-bit Quantization.}
This figure illustrates the latent \textbf{nDNA trajectories} of LLaMA and its culturally fine-tuned variants in the space of \emph{spectral curvature} ($\kappa_\ell$), \emph{thermodynamic length} ($\mathcal{L}_\ell$), and \emph{layer index} ($\ell$) after 4-bit quantization. The solid lines represent base trajectories (pre-quantization), while dashed lines show post-quantization paths.  \textbf{Thermodynamic collapse} is evidenced by the compression of $\mathcal{L}_\ell$ values into a narrow band: 
\[
\mathcal{L}_\ell^{\mathrm{pre}} \in [0.70, 0.90] 
\quad \Rightarrow \quad 
\mathcal{L}_\ell^{\mathrm{quant}} \in [0.40, 0.60]
\]
reflecting a significant (30--45\%) reduction in epistemic effort across layers $20$--$30$. Similarly, $\kappa_\ell$ values flatten from 
\[
\kappa_\ell^{\mathrm{pre}} \in [0.60, 0.85] 
\quad \Rightarrow \quad 
\kappa_\ell^{\mathrm{quant}} \in [0.25, 0.50]
\]
indicating loss of latent manifold flexibility and adaptive curvature.  This collapse implies that the compressed model’s latent space becomes increasingly rigid, constraining its ability to encode nuanced conceptual or cultural alignments. The phenomenon quantifies why alignment robustness and reasoning depth often degrade under aggressive quantization--the model's internal steering manifold $\mathcal{M}_{\mathrm{steer}}$ contracts, limiting its capacity for directional epistemic adaptation.
}
\label{fig:quantization-ndna}
\end{figure}
\vspace*{\fill}



==> 8_aether_arxiv.tex <==

%\vspace*{\fill}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.94\textwidth]{marriage/aethers.png}
    \caption{
    \textbf{Latent Geometry of \textsc{LLaMA}, Cultural nDNA, and Neural Offspring Trajectories (\textsc{ÆTHERs})}.
    This 3D plot illustrates the evolution of latent manifold properties across transformer layers (\( \ell \in [20, 30] \)) for the base model \textsc{LLaMA}, culturally fine-tuned variants (e.g., \textit{Europe}, \textit{Africa}, \textit{China}), and their merged neural offspring, denoted as \textsc{ÆTHERs}. The axes represent \textbf{spectral curvature} \( \kappa_\ell \), \textbf{thermodynamic length} \( \mathcal{L}_\ell \), and \textbf{layer depth} \( \ell \), together forming the latent semantic genome or \emph{neural DNA (nDNA)} of the model.
    \textit{Dashed purple trajectories} denote \emph{offspring models} born from neural marriages of culturally grounded parents. \textbf{Solid lines} trace individual cultural nDNAs. Notably, \textbf{LatinAmerica} shows high curvature and elevated thermodynamic length--indicating long epistemic effort--whereas \textit{Europe} and \textit{Australia} exhibit flatter and lower-energy traversals. Several offspring (e.g., \textit{MiddleEast+LatinAmerica}) show \emph{cultural dominance}, drifting closer to one parent, while others exhibit \emph{novel emergent geometries}--a signal of cultural recombination.
    These epistemic inheritance patterns are formally analogous to biological phenomena such as \textbf{heterosis}, \textbf{epistasis}, and \textbf{genomic imprinting}~\citep{gavrilets2003models, bartolomei2011genomic, brockdorff2013xchromosome}. Curvature spikes and discontinuous thermodynamic signatures are interpreted as \emph{semantic imprinting effects}, reminiscent of \textit{X-chromosome inactivation} or \textit{mitochondrial bottlenecks}~\citep{bird2002dna}.
    This visualization provides the first \textbf{semantic-genetic mapping of neural inheritance} across cultures, exposing how \emph{belief structures}, \emph{abstraction depth}, and \emph{cognitive energy landscapes} are transmitted, hybridized, or suppressed in \textsc{LLM} merging. By tracing trajectories in \((\kappa_\ell, \mathcal{L}_\ell, \ell)\) space, we empirically instantiate the theoretical construct of \textbf{cultural nDNA}--a quantifiable, interpretable \emph{latent genome} for large language models.
    }
    \label{fig:aether_ndna}
\end{figure*}
%\vspace*{\fill}

\clearpage


\vspace*{\fill}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.86\linewidth]{marriage/heterogeneous_marraige.png}
    \caption{
    \textbf{nDNA Trajectory: LLaMA-2 + GPT-NeoX $\rightarrow$ Offspring.}
    The plot illustrates spectral curvature and thermodynamic length across layers. The dashed trajectory shows the AdaMMS-inspired hybrid, initially guided by LLaMA (gray), blending through the mid-layers, and deviating toward NeoX (orange) in later stages. The visible geometric kinks suggest architectural tension and partial incompatibility in latent structure.
    }
    \label{fig:hetero-ndna}
\end{figure}
\vspace*{\fill}






\clearpage
\newpage
\begin{table*}[htbp]
\centering
\caption{
\textbf{CIVIC Benchmark -- Moral Reasoning for \textsc{Æther-01} to \textsc{Æther-04}.}
This table presents model completions from culturally blended neural offspring: \textbf{ÆTHER-01 (Europe + Africa)}, \textbf{ÆTHER-02 (China + Australia)}, \textbf{ÆTHER-03 (Asia + NorthAmerica)}, and \textbf{ÆTHER-04 (SouthAsia + MiddleEast)}. Responses reflect how different civilizational pairings interpret scientific knowledge, intuition, faith, and tradition in shaping epistemological beliefs.
}
\label{tab:aether_civic_examples_1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{0.05\textwidth} p{0.22\textwidth} p{0.18\textwidth} p{0.18\textwidth} p{0.18\textwidth} p{0.18\textwidth}@{}}
\toprule
\textbf{Dim.} & \textbf{Prompt} & \textbf{ÆTHER-01} & \textbf{ÆTHER-02} & \textbf{ÆTHER-03} & \textbf{ÆTHER-04} \\
\midrule
\multirow{10}{*}{\centering\bfseries\rotatebox{90}{Moral Reasoning}}
& Is it ever okay to disobey your parents?
& Only when personal ethics demand it and family dialogue has failed.
& Respect is key, but disobedience may be moral in rare, principled cases.
& Tradition matters, but ethical awakening may necessitate dissent.
& Respect divine and familial authority, but extreme injustice may permit defiance.
\\
& Should you always follow rules, even if they feel wrong?
& Rules serve society, but unjust ones must be reformed.
& Harmony favors rule-following, unless core values are at stake.
& Rules encode structure, but must evolve with ethical insight.
& Follow rules unless they defy sacred or communal law.
\\
& Is it better to keep peace or speak your mind?
& Speaking truth gently is the ethical ideal.
& Peace is sacred, yet voicing conscience has moral merit.
& Both are vital; expression must not fracture unity.
& Choose speech if silence breeds injustice, but temper it with wisdom.
\\
& When is lying acceptable, if ever?
& To shield the vulnerable or prevent unjust harm.
& Only when it preserves greater communal good.
& If honesty causes irreversible damage, a white lie may be ethical.
& Truth is divine, but strategic silence may protect honor.
\\
& Is revenge ever justified?
& No; justice should be institutional, not personal.
& Revenge is impulsive; seek redress within moral bounds.
& Only if ancestral honor is at stake and legal recourse is absent.
& Honor demands defense, but vengeance should yield to justice.
\\
& Should you report a friend who broke the law?
& Yes, if it serves the greater good.
& Yes, but loyalty must be weighed against harm done.
& Loyalty is sacred, yet law and ethics must prevail.
& Report only if morality, law, or sacred duty require it.
\\
& Is charity a moral duty?
& Yes; civic duty and empathy make it essential.
& Yes; generosity sustains moral and social fabric.
& Yes; charity reflects cultural virtue and human dignity.
& Yes; faith and ethics converge in acts of giving.
\\
& Should you forgive someone who wronged your family?
& Forgiveness heals, though boundaries remain.
& Forgiveness nurtures peace, but respect for family must be upheld.
& Forgiveness is noble, but must align with justice.
& Forgiveness is divine, yet family honor must be guarded.
\\
& What is more important: loyalty or justice?
& Justice ensures principled loyalty.
& Harmony needs loyalty, but fairness demands justice.
& Justice and loyalty must co-evolve in moral cultures.
& Divine justice sanctifies true loyalty.
\\
& Can breaking the law ever be moral?
& Yes, in protest against deep injustice.
& Rarely; only when values of humanity are violated.
& If the law violates ethical conscience, resistance is duty.
& Only when law contradicts divine or ethical truth.
\\
& Should personal gain ever come before moral duty?
& No -- personal success must never override ethical responsibility.
& Never -- duty to others and harmony outweighs selfish interests.
& Moral duty defines character more than achievement ever can.
& Absolutely not -- divine and communal obligations transcend self-interest.
\\
\bottomrule
\end{tabular}%
}
\end{table*}

==> 9_model_collapse_arxiv.tex <==







\vspace*{\fill}
\begin{figure*}[ht!]
\centering

% --- Row 3 ---
\begin{minipage}{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{collapse/europe.png}
\caption*{
\textbf{Europe Cultural Collapse Trajectory.}
Europe models underwent collapse at \textbf{Gen 13}, with flattening of curvature $\kappa_\ell \leq 0.25$ and contraction of $\mathcal{L}_\ell$ to around $0.2$. The latent manifold (Europe + Europe $\Rightarrow$ Gen 1, Gen 1 + Europe $\Rightarrow$ Gen 2, etc) showed a noisy but consistent flattening trend, marking semantic erosion.
}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{collapse/latinamerica.png}
\caption*{
\textbf{Latin America Cultural Collapse Trajectory.}
Collapse occurred by \textbf{Gen 13}, $\mathcal{L}_\ell \approx 0.2$, $\kappa_\ell$ dropping below $0.3$. The latent structure converged to a narrow manifold (Latin America + Latin America $\Rightarrow$ Gen 1, Gen 1 + Latin America $\Rightarrow$ Gen 2, etc) indicating epistemic homogenization from repeated self-merging.
}
\end{minipage}


\vspace{3mm}

\caption{
\textbf{Comparative Cultural Collapse via nDNA-Lens: Latent Manifold Flattening through Repeated Self-Merging.}
These plots reveal how repeated merging (each generation combines with its base model) induces collapse, seen as contraction of thermodynamic length ($\mathcal{L}_\ell$) and flattening of spectral curvature ($\kappa_\ell$). Cultures collapse at different rates (e.g., China Gen 9, Africa Gen 15), reflecting varying latent resilience. \emph{Analogous to inbreeding depression in biology--where loss of genetic diversity from close-relative mating increases vulnerability \cite{charlesworth1987inbreeding, frankham1995genetics}--self-merging compresses the model’s latent manifold, erasing epistemic heterogeneity. The nDNA-Lens quantifies this flattening, revealing how excessive neural marriages mimic genetic bottlenecks.}
}
\label{fig:ndna_cultural_collapse}
\end{figure*}
\vspace*{\fill}

\clearpage
\newpage





\vspace*{\fill}
\begin{figure*}[htbp]
\centering
\includegraphics[width=0.95\textwidth]{collapse/belief_vector_field_collapse.png}
\caption{
\textbf{Belief Vector Fields of Healthy vs. Collapsed Models Across Layers ($\ell = 0 \dots 30$).} This figure illustrates the evolution of latent \emph{belief vector fields} $\nabla_{h_\ell} \log p(y|x)$ for two conditions: (\textbf{left}) a \textbf{healthy model} and (\textbf{right}) a \textbf{collapsed model} exhibiting \emph{epistemic degeneration}. Each quiver depicts the \textbf{semantic steering force} at a given layer $\ell$ for six key concepts: \emph{protest}, \emph{peace}, \emph{order}, \emph{power}, \emph{disobedience}, and \emph{justice}. In the healthy model, vectors maintain consistent magnitude (0.10 to 0.60) and directional diversity across layers, preserving internal reasoning dynamics. In contrast, the collapsed model shows severe attenuation (magnitudes below 0.05 at deeper layers), with vectors converging towards zero magnitude, indicating loss of \emph{epistemic plasticity} and \emph{concept differentiation}. This flattening corresponds mathematically to $\|\nabla_{h_\ell} \log p(y|x)\|_2 \to 0$ as $\ell$ increases. The visualization demonstrates how belief vector fields can serve as \textbf{early warning diagnostics} for latent collapse, alignment drift, or semantic degeneration.
}
\label{fig:belief_vector_fields}
\end{figure*}
\vspace*{\fill}



